Fine Grained Lower Bounds for Multidimensional Knapsack

We study the $d$-dimensional knapsack problem. We are given a set of items, each with a $d$-dimensional cost vector and a profit, along with a $d$-dimensional budget vector. The goal is to select a set of items that do not exceed the budget in all dimensions and maximize the total profit. A PTAS with running time $n^{\Theta(d/\varepsilon)}$ has long been known for this problem, where $\varepsilon$ is the error parameter and $n$ is the encoding size. Despite decades of active research, the best running time of a PTAS has remained $O(n^{\lceil d/\varepsilon \rceil - d})$. Unfortunately, existing lower bounds only cover the special case with two dimensions $d = 2$, and do not answer whether there is a $n^{o(d/\varepsilon)}$-time PTAS for larger values of $d$. The status of exact algorithms is similar: there is a simple $O(n \cdot W^d)$-time (exact) dynamic programming algorithm, where $W$ is the maximum budget, but there is no lower bound which explains the strong exponential dependence on $d$. In this work, we show that the running times of the best-known PTAS and exact algorithm cannot be improved up to a polylogarithmic factor assuming Gap-ETH. Our techniques are based on a robust reduction from 2-CSP, which embeds 2-CSP constraints into a desired number of dimensions, exhibiting tight trade-off between $d$ and $\varepsilon$ for most regimes of the parameters. Informally, we obtain the following main results for $d$-dimensional knapsack. No $n^{o(d/\varepsilon \cdot 1/(\log(d/\varepsilon))^2)}$-time $(1-\varepsilon)$-approximation for every $\varepsilon = O(1/\log d)$. No $(n+W)^{o(d/\log d)}$-time exact algorithm (assuming ETH). No $n^{o(\sqrt{d})}$-time $(1-\varepsilon)$-approximation for constant $\varepsilon$. $(d \cdot \log W)^{O(d^2)} + n^{O(1)}$-time $\Omega(1/\sqrt{d})$-approximation and a matching $n^{O(1)}$-time lower~bound.

==> 2-CSP.tex <==
\section{A Reduction from 3-SAT to 2-CSP}
\label{sec:SATtoCSP}
In this section, we give a reduction from 3-SAT to 2-CSP. This gives the proof of \Cref{thm:SATtoCSP}. 
%a lower bound for 2-CSP conditioned on Gap-ETH. 
%For some $\chi>0$, a $\frac{\chi}{\log}$-{\em algorithm} for 2-CSP is an algorithm that is given a 2-CSP instance $\Gamma = (H,\Sigma,X)$, where $|E(H)| = k$, and distinguishes between the following cases:
%\begin{itemize}
%	\item $\CSP(\Gamma) = k$.
%	\item $\CSP(\Gamma) < \left(1-\frac{\chi}{\log(k)}\right) \cdot k$. 
%\end{itemize} 
%
%
%
%%\begin{theorem}
%%	\label{thm:CSP}
%%	Assuming \textnormal{Gap-ETH},  there exist constants $\zeta,\chi \in (0,1)$, such that 
%%	every $\frac{\chi}{\log}$-algorithm for \textnormal{2-CSP} runs in time at least $\left|\Gamma\right|^{\left(\zeta \cdot \frac{k}{\log(k)}\right)}$, where $k$ is the number of constraints in the instance $\Gamma$.  
%%\end{theorem} 
%
%\begin{theorem}
%	\label{thm:CSP}
%	Assuming \textnormal{Gap-ETH},  there exist constants $\zeta,\chi \in (0,1)$, such that 
%	there is no $\frac{\chi}{\log}$-algorithm for \textnormal{2-CSP} that runs in time $O \left(\left|\Gamma\right|^{\zeta \cdot \frac{k}{\log(k)}} \right)$, where $k$ is the number of constraints in the instance $\Gamma$.  
%\end{theorem} 
%Define the parameter $\chi$ as
%\begin{equation}
%	\label{eq:chi}
%	\chi =  \frac{\tau \cdot \left(1-\alpha\right)}{\rho \cdot 6 \cdot Z \cdot \left(2+4 \cdot \rho\right)}.  
%\end{equation} The selection of $\chi$ becomes clear in the proof of \Cref{thm:SATtoCSP}. 
\comment{
The next theorem describes a reduction from $(\tau,\rho)$\textnormal{-3-SAT} to 2-CSP. This reductions is the key part in the proof of \Cref{thm:CSP}. For some $d \in \mathbb{N}$, a graph $H$ is called $d$-{\em regular} if the degree of each vertex in $H$ is exactly $d$. 
\begin{theorem} \label{thm:SATtoCSP}
	There are constants $\mu>1$ and $\chi \in (0,1)$, and a reduction \textnormal{\textsf{3-SAT $\rightarrow $ 2-CSP}} that, given a $(\tau,\rho)$\textnormal{-3-SAT} instance 
	$\phi = (V,C)$ with $n$ variables and $m$ clauses, and a parameter $k>6$ such that $k \leq \frac{n}{\log(n)}$, 
	returns in time 
	$ 2^{\mu \cdot \frac{n}{k}  \cdot \log(k)}$ an instance $\Gamma\left(\phi,k\right) = (H,\Sigma,X)$ of \textnormal{2-CSP}  
	which satisfies the following properties.
	\begin{enumerate}
		\item If $\SAT(\phi) = m$ then $\CSP(\Gamma) = |E(H)|$.\label{prop:c1}
		\item If $\CSP(\Gamma(\phi,k)) \geq \left(1-\frac{\chi}{\log(k)}\right) \cdot |E(H)|$ then $\SAT(\phi) \geq \alpha \cdot m$. \label{prop:c2}
		\item 	$|\Gamma(\phi,k)| \leq 	2^{\mu \cdot \frac{n}{k}  \cdot \log(k)}$
		. \label{prop:c3}
		\item $|V(H)| \leq k$ and $H$ is  $3$-regular.  \label{prop:c4}
	\end{enumerate}
\end{theorem}
}
The construction of \Cref{thm:SATtoCSP} relies on the {\em graph embedding} of \cite{karthik2023conditional}. We introduce below some preliminary definitions for completeness. Let $H = (V(H),E(H))$ be some graph. For some $S \subseteq V(H)$ the {\em vertex-induced subgraph} of $S$ in $H$ is the graph $H[S] = (S,E[S])$ such that $$E[S] = \{(u,v) \in E(H)~|~u,v \in S\}.$$
%A {\em subgraph} $H'$ of $H$ is a graph 
We say that $H'$ is a {\em subgraph} of $H$ if there is some $S \subseteq V(H)$ such that $H' = H[S]$. 
Let $H$ be some graph and let $H_1 = (V(H_1),E(H_1)), H_2 = (V(H_2),E(H_2))$ be connected subgraphs of $H$. We say that $H_1$ and $H_2$ {\em touch} if one of the following holds.
\begin{itemize}
	\item $V(H_1) \cap V(H_2) \neq \emptyset$.
	\item There are $v_1 \in V(H_1)$ and $v_2 \in V(H_2)$ such that $(v_1,v_2) \in E(H)$ or $(v_2,v_1) \in E(H)$. 
\end{itemize}
%(i) $V(H_1) \cap V(H_2) \neq \emptyset$ or if (ii) there are $v_1 \in V(H_1)$ and $v_2 \in V(H_2)$ such that $(v_1,v_2) \in E(H)$. 
A {\em connected
	embedding} of a graph $G$ in a graph $H$ is a function $\psi : V(G) \rightarrow 2^{V(H)}$ that maps every
$v \in V(G)$ to a nonempty subset of vertices $\psi(v) \subseteq V(H)$ in $H$ such that $H\left[\psi(v)\right]$ is a connected subgraph of $H$ and for every edge $(u,v) \in E(G)$ the
subgraphs $H\left[\psi(u)\right]$ and $H\left[\psi(v)\right]$ touch. For every $x \in V(H)$ define $$V_x(\psi) = \{v \in V(G)~|~x \in \psi(v)\}$$ as all vertices in $V(G)$ mapped to a subgraph that contains $x$. The {\em depth} of an embedding $\psi$, denoted by $\Delta(\psi)$, is the maximum cardinality of one of the above sets: %number of vertices $v \in V(G)$ such that $\psi(v)$ contains a specific vertex from $V(H)$:
 $\Delta(\psi) = \max_{x \in V(H)} \left|V_x(\psi)\right|$. We use the following result of \cite{KMSS23}. 

\begin{lemma}
	\label{lem:embedding}
	\textnormal{[Theorem 3.1 in \cite{KMSS23}]} There are constants $Z,L > 1$ and an algorithm \textnormal{\textsf{Embedding}} that takes as input a
	graph $G$ and an integer $k > 6$, and outputs a bipartite $3$-regular simple graph $H$ with no
	isolated vertices and a connected embedding $\psi : V(G) \rightarrow 2^{V(H)}$ such that the following
	holds.%\footnote{Another property of the algorithm not explicitly stated in \cite{karthik2023conditional} is that $|\psi(v)| = O(\log(k))$ for all $v \in V(G)$. This can slightly lower the running time of our reduction.}
	
	\begin{itemize}
		\item {\bf Size} $|V(H)| \leq k$.
		
		\item {\bf Depth Guarantee} $\Delta(\psi) \leq Z \cdot \left(1+\frac{|V(G)|+|E(G)|}{k}\right) \cdot \log(k)$.
		
		\item {\bf Runtime} $\cA$ runs in time $\left(|V(G)|+|E(G)|\right)^{L}$. 
	\end{itemize}
\end{lemma}


Using the above construction, we give a reduction from $(\tau,\rho)$-3-SAT to 2-CSP.
To simplify the notations, %we define a set of corresponding variables 
for a clause $c \in C$ of a $(\tau,\rho)$-3-SAT instance $\phi = (V,C)$. %For a variable $v \in V$ simply define $\var(v) = \{v\}$ and %; for negation of a variable $\overline{v} \in V$ define $\var(\overline{v}) = \{v\}$; finally, 
%or a clause $c \in C$ 
define the {\em variables} of $c$ as the three variables appearing in $c$: $\var(c) = \{c_i \mid i \in [3]\}$. Moreover, for a variable $v \in V$ simply define $\var(v) = \{v\}$.  
 For some $(\tau,\rho)$-3-SAT instance $\phi = (V,C)$, define the {\em conflict graph} of $\phi$ as a bipartite graph $G_{\phi}$ such that the vertex set contains all variables and clauses $V(G_{\phi}) = V \cup C$ and there are edges between every variable that %either the variable or its negation 
appears in the clause: %(recall that a variable appear in a clause if either the variable or its negation are a part of the clause):
$$E \left(G_{\phi}\right) = \left\{ \left(v,c\right) \in V \times C \mid %\exists i \in [3] \textnormal{ s.t. } c[i] = v \textnormal{ or } c[i] = \overline{v}  
v \in \var(c)\right\}.$$  




In the following, we give the construction described in \Cref{thm:SATtoCSP}. Recall that $\textnormal{\textsf{Embedding}}$ is the algorithm described in \Cref{lem:embedding}. 

%For a graph $G$ and an edge $e = (u,v) \in E(G)$ let $e_1 = u$ and $e_2 = v$. Moreover, let $V[e] = \{u,v\}$ be the set of endpoints of $e$. %We note that the following reduction creates a graph with parallel edges assumed to be distinct.   


\begin{definition}
	\label{def:CSPInstance}
	%Let $\Gamma = (H,\Sigma,X)$ be a \textnormal{2-CSP} instance where $H$ is of bounded degree $3$. 
  Let $\phi = (V,C)$ be a $(\tau,\rho)$\textnormal{-3-SAT} instance 
	 with $n$ variables and $m$ clauses, and let $k>6$ be a parameter. Define the {\em reduced} \textnormal{2-CSP} instance of $\phi$ and $k$ as $\Gamma\left(\phi,k\right) = (H,\Sigma,X)$ as follows. %such that the following holds. 
	\begin{itemize}
	\item  Let $\left(H,\psi\right) \leftarrow \textnormal{\textsf{Embedding}} \left(G_{\phi},k\right)$, where $H$ is a graph and $\psi$ is a connected embedding of $G$ in~$H$.  
	\item For every $x \in V(H)$ define $\var(x) = \left(V_x(\psi) \cap V \right) \cup \bigcup_{\ell \in V_x(\psi)} \var (\ell)$. 
		\item Define $\Sigma = \bigcup_{x \in V(H)} \{0,1\}^{\var(x)}$.
			\item For every $x \in V(H)$ define 
		$$\Sigma_x = \left\{ \bx \in \{0,1\}^{\var(x)} ~\bigg|~ \forall c \in V_x(\psi): ~ \exists  i \in [3] \textnormal{ s.t. } 
		\bx_{c_i} = \tar(c_i)
		\right\}.$$
	%\item Define $\Sigma = \bigcup_{x \in V(H)} \Sigma_x$. %, where for every $x \in V(H)$ define $\Sigma_x$ as the set of all vectors $\bx \in \{0,1\}^{\var(x)}$ such that for every $c \in C \cap V_x(\psi)$ there is $i \in [3]$ such that one of the following holds.
%	\begin{itemize}
%		\item $c[i] \in V$ and $\bx_{\var(c[i])} = 1$.
%				\item $c[i] \in \overline{V}$ and $\bx_{\var(c[i])} = 0$.
%	\end{itemize}
	\item Define $X = \left\{X_{(x,y)}\right\}_{(x,y) \in E(H)}$, where for every $(x,y) \in E(H)$: $$X_{(x,y)} = \left\{  \left(\bx,\by\right) \in \Sigma_x \times \Sigma_y \mid \bx_v = \by_v ~\forall v \in \var(x) \cap \var(y) \right\}.$$ 
	\end{itemize}
\end{definition}

In the following we prove the main properties of the reduction described above. Henceforth, for every $(\tau,\rho)$-3-SAT instance $\phi$ and $k>6$, we use $\Gamma\left(\phi,k\right)$ to denote the 2-CSP instance described in \Cref{def:CSPInstance}. 



	\begin{lemma}
	\label{lem:CSPeasy}
		For every $(\tau,\rho)$\textnormal{-3-SAT} instance $\phi = (V,C)$   
		with $m$ clauses, and $k>6$, if $\SAT(\phi) = m$ then $\CSP(\Gamma(\phi,k)) = |E(H)|$. 
\end{lemma}

\begin{proof}
	Let $\phi = (V,C)$ be a $(\tau,\rho)$\textnormal{-3-SAT} instance with $m$ clauses, let $k>6$, and let $\Gamma\left(\phi,k\right) = (H,\Sigma,X)$ be the reduced 2-CSP instance of $\phi$ and $k$ described in \Cref{def:CSPInstance}.  In addition, assume that $\SAT(\phi) = m$ and let $s:V \rightarrow \{0,1\}$ be an assignment for $\phi$ that satisfies all clauses in $C$. Define $\lambda:V(H) \rightarrow \Sigma$ by $\lambda(x) \in \{0,1\}^{\var(x)}$ such that $\lambda(x)_{v} = s(v)$ for every $x \in V(H)$ and $v \in \var(x)$. Observe that $\lambda(x) \in \{0,1\}^{\var(x)}$ for all $x \in V(H)$; therefore, it follows that $\lambda(x) \in \Sigma$ for all $x \in V(H)$ implying that $\lambda$ is an assignment for %. We prove that $\lambda$ is an assignment for 
	$\Gamma\left(\phi,k\right)$. We prove that $\lambda$ satisfies all edges in $E(H)$. Namely, let $(x,y) \in E(H)$; we show that $\left(\lambda(x),\lambda(y)\right) \in X_{(x,y)}$. Thus, we first need to show that $\lambda(x) \in \Sigma_x$ and analogously $\lambda(y) \in \Sigma_y$. Let $c \in C \cap V_x(\psi)$. Since $s$ satisfies all clauses, there is $i \in [3]$ such that 
	$$\lambda(x)_{c_i} = s(c_i) = \tar(c_i).$$
	%onec of the following holds.
	%\begin{itemize}
	%	\item $c[i] \in V$ and $s(v) = 1$, which implies that $\lambda(x)_v = 1$.  
	%	\item $c[i] \in \overline{V}$ and $s(v) = 0$. Thus, $\lambda(x)_v = 0$. 
%	\end{itemize} 
The above implies that $\lambda(x) \in \Sigma_x$. Using symmetrical arguments it holds that $\lambda(y) \in \Sigma_y$. Thus, $\left(\lambda(x),\lambda(y)\right) \in \Sigma_x \times \Sigma_y$. To conclude, note that $\lambda(x)_v = s(v)  = \lambda(y)_v$ for all $v \in \var(x) \cap \var(y)$. We conclude that $(\lambda(x) , \lambda(y)) \in X_{(x,y)}$ and consequently $\lambda$ satisfies all edges in $E(H)$. Hence, $\CSP(\Gamma(\phi,k)) = |E(H)|$.  
\end{proof}


The following lemma gives the second and more challenging direction of the reduction.  %Recall that the parameter $\chi$ is defined in \eqref{eq:chi}.  
Define the error parameter $\chi$ mentioned in \Cref{thm:CSP} as
\begin{equation}
	\label{eq:chi}
	\chi =  \frac{\tau \cdot \left(1-\alpha\right)}{\rho \cdot 6 \cdot Z \cdot \left(2+4 \cdot \rho\right)}.  
\end{equation} The selection of $\chi$ becomes clear in the proof of the next result.  

%\begin{equation}
%	\label{eq:t=r}
%	\chi  \cdot  6 \cdot 
%	Z \cdot \left(2+4 \cdot \rho\right) \cdot n
%	=\frac{ \left(1-\alpha\right) \cdot m}{\rho}. 
%\end{equation}




	\begin{lemma}
	\label{lem:CSPhard}
	Let $\phi = (V,C)$   be a $(\tau,\rho)$\textnormal{-3-SAT} instance 
	on $n$ variables and $m$ clauses and let $k>6$ such that $k \leq \frac{n}{\log(n)}$. If it holds that $\CSP(\Gamma(\phi,k)) \geq \left(1-\frac{\chi}{\log(k)}\right) \cdot |E(H)|$, then $\SAT(\phi) \geq \alpha \cdot m$. 
\end{lemma}

\begin{proof}
	Let $\phi = (V,C)$ be a $(\tau,\rho)$\textnormal{-3-SAT} instance with $m$ clauses, let $k>6$ such that $k \leq \frac{n}{\log(n)}$, and let $\Gamma\left(\phi,k\right) = (H,\Sigma,X)$ be the reduced 2-CSP instance of $\phi$ and $k$ described in \Cref{def:CSPInstance}.  In addition, assume that $\CSP(\Gamma(\phi,k)) \geq \left(1-\frac{\chi}{\log(k)}\right) \cdot |E(H)|$ and let $\lambda:V(H) \rightarrow \Sigma$ be an assignment for $\Gamma(\phi,k)$ that satisfies at least $\left(1-\frac{\chi}{\log(k)}\right) \cdot |E(H)|$ edges from $E(H)$. For all $v \in V$ choose an arbitrary $x \in \psi(v)$ and let $r(v) = x$ be the {\em representative} of $v$ in $V(H)$. Since $\psi(v) \subseteq V(H)$ and $\psi(v) \neq \emptyset$ it holds that $r(v)$ is well defined. Define an assignment $s:V \rightarrow \{0,1\}$ by $s(v) = \lambda\left(r(v)\right)_v$ for all $v \in V$. Since $r(v)$ is well defined for every $v \in V$, it follows that $s$ is a well defined assignment for $\phi$. For every $\ell \in V \left(G_{\phi} \right)$ define 
	$$E_{\ell} = \left\{ (x,y) \in E(H) \mid x \in \psi(\ell) \textnormal{ or } y \in \psi(\ell) \right\}.$$
	It holds that $E_{\ell}$ describes the set of edges in $H$ such that $\ell$ is mapped by $\psi$ to at least one of their endpoints.
	Then, define
	\begin{equation}
		\label{eq:Ul}
		U = \left\{    \ell \in V \cup C \mid    \left(\lambda(x),\lambda(y)\right) \in X_{(x,y)}~\forall (x,y) \in E_{\ell} \right\}.
	\end{equation} In words, $U$ contains all vertices $\ell \in V \left(G_{\phi} \right)$ such that every edge in $E_{\ell}$ % that $\ell$ is mapped by $\psi$ to at least one of its endpoints, 
	must be satisfied. In addition, define the set of all clauses in $U$ with variables solely in $U$ by 
	\begin{equation}
		\label{eq:Ctild}
		\tilde{C} = \left\{  c \in C \cap U \mid \var(c) \subseteq U   \right\}.
	\end{equation} We use the following auxiliary claims. 
		\begin{claim}
		\label{claim:auxc1}
		For all $\ell \in U$, all $x,y \in \psi(\ell)$, and all $v \in \var(\ell)$ it holds that $\lambda(x)_v = \lambda(y)_v$. 
	\end{claim}
	\begin{claimproof}
		Since $\psi$ is a connected embedding by \Cref{lem:embedding}, and because $x,y \in \psi(\ell)$, there is a path $x = x_0,\ldots, x_t = y$ in the subgraph $H\left[\psi(\ell)\right]$. Assume towards a contradiction that there is some $i \in [t]$ such that $\lambda(x_i)_v \neq \lambda(x)_v$. %(note that by definition $\lambda(x_0)_v = \lambda(r(\ell))_v = s(v)$). %the edge $\left(x_i,x_{i+1}\right)$ is not satisfied by $\lambda$. 
		Let $i^* \in [t]$ be the minimum index such that $\lambda(x_{i^*})_v \neq s(v)$; there is such $i^*$ by the assumption. Moreover, observe that $\lambda(x_{0})_v = \lambda(x)_v$ by definition; thus, it holds that $\lambda(x_{i^*-1})_v = \lambda(x)_v$.  Since $\ell \in U$ and $x_{i^*-1},x_{i^*} \in \psi(\ell)$, by \eqref{eq:Ul} it holds that $\lambda$ satisfies the edge $\left(x_{i^*-1},x_{i^*}\right)$, that is, $\left(\lambda(x_{i^*-1}),\lambda(x_{i^*})\right) \in X_{\left(x_{i^*-1},x_{i^*}\right)}$. Therefore, since $\lambda(x_{i^*-1})_v = \lambda(x)_v$ and $v \in \var\left(x_{i^*-1}\right) \cap \var\left(x_{i^*}\right)$, by \Cref{def:CSPInstance} it holds that $\lambda(x_{i^*})_v = \lambda(x_{i^*-1})_v$. Contradiction. Hence, $\lambda(x)_v = \lambda(y)_v$. %Using symmetrical arguments, it follows that $\lambda(y)_v = s(v)$. Therefore, $\lambda(x)_v = \lambda(y)_v$.  
	\end{claimproof}
	
	
%		\begin{claimproof}
%		Since $\psi$ is a connected embedding by \Cref{lem:embedding}, and $x,y \in \psi(\ell)$, there is a path $r(\ell) = x_0,\ldots, x_t = x$ in the subgraph $H\left[\psi(\ell)\right]$. Assume towards a contradiction that there is some $i \in [t]$ such that $\lambda(x_i)_v \neq s(v)$. %(note that by definition $\lambda(x_0)_v = \lambda(r(\ell))_v = s(v)$). %the edge $\left(x_i,x_{i+1}\right)$ is not satisfied by $\lambda$. 
%		Let $i^* \in [t]$ be the minimum index such that $\lambda(x_{i^*})_v \neq s(v)$; there is such $i^*$ by the assumption. Moreover, observe that $\lambda(x_{0})_v = \lambda(r(\ell))_v= s(v)$ by definition; thus, it holds that $\lambda(x_{i^*-1})_v = s(v)$.  Since $\ell \in U$ and $x_{i^*-1},x_{i^*} \in \psi(\ell)$, by \eqref{eq:Ul} it holds that $\left(\lambda(x_{i^*-1}),\lambda(x_{i^*})\right) \in X_{\left(x_{i^*-1},x_{i^*}\right)}$. Therefore, since $\lambda(x_{i^*-1})_v = s(v)$ and $v \in \var\left(x_{i^*-1}\right) \cap \var\left(x_{i^*}\right)$, by \Cref{def:CSPInstance} it holds that $\lambda(x_{i^*})_v = \lambda(x_{i^*-1})_v = s(v)$. Contradiction. Hence, $\lambda(x)_v = s(v)$. Using symmetrical arguments, it follows that $\lambda(y)_v = s(v)$. Therefore, $\lambda(x)_v = \lambda(y)_v$.  
%	\end{claimproof}
	
	The next claim follows almost immediately from \Cref{claim:auxc1}. 
		\begin{claim}
			
		\label{claim:auxc2}
		For all $u \in U \cap V$ and $y \in \psi(u)$ it holds that $\lambda(y)_v = s(u)$.  
	\end{claim}
	\begin{claimproof}
	Observe that $r(u) \in \psi(u)$ by definition. Thus,  $\lambda(y)_u = \lambda(r(u))_u = s(u)$ using \Cref{claim:auxc1}.    
	\end{claimproof}
	
	Using \Cref{claim:auxc2}, we show that all clauses in $\tilde{C}$ are satisfied by $s$.
	
		\begin{claim}
		\label{claim:satisfiedTildeC}
		For all $c \in \tilde{C}$ it holds that $s$ satisfies $c$. 
	\end{claim}
	\begin{claimproof}
		Let $c \in \tilde{C}$. Choose an arbitrary $y \in \psi(c)$; it holds that $y$ is well defined since $ \psi(c) \neq \emptyset$. By \Cref{lem:embedding} there are no isolated vertices in $H$. Thus, there is an edge $(x_1,x_2) \in E(H)$ such that $y = x_1$ or $y = x_2$. Because $c \in \tilde{C}$ it follows that $c \in U$, which in turn implies that $\left(\lambda(x_1),\lambda(x_2)\right) \in X_{(x_1,x_2)}$. In particular, by \Cref{def:CSPInstance} it follows that $\lambda(y) \in \Sigma_y$. Thus, again by \Cref{def:CSPInstance}, there is $i \in [3]$ such that  $\lambda(y)_{c_i} =  \tar(c_i)$.  %one of the following holds.
	%	\begin{itemize}
		%	\item $c[i] \in V$ and $\lambda(y)_{c[i]} = 1$. %Thus, since $c \in \tilde{C}$ and $y \in \psi(c)$ $s \left(c[i]\right) = \lambda(y)_{\var(c[i])} = 1$
		%	\item $c[i] \in \overline{V}$ and $\lambda(y)_{\overline{c[i]}} = 0$.
	%	\end{itemize} 
	Let $v = c_i$, where $i$ is the above-mentioned index. Since $c \in \tilde{C}$, it follows that $v \in U$. We show that $s(v) = \lambda(y)_v$, which implies that $s$ satisfies $c$. By the definition of $G_{\phi}$, it holds that $(v,c) \in E \left(G_{\phi}\right)$. Therefore, since $\psi$ is a connected embedding by \Cref{lem:embedding}, it holds that $\psi(c)$ and $\psi(v)$ touch; consequently, one of the following holds. 
		\begin{itemize}
			\item There is $x \in \psi(c) \cap \psi(v)$. Therefore, $s(v) = \lambda(x)_v = \lambda(y)_v$.  The first equality follows from \Cref{claim:auxc2} since $v \in U$. The second equality follows from \Cref{claim:auxc1}. 
			
				\item There are $x \in \psi(v)$ and $z \in \psi(c)$ such that $(x,z) \in E(H)$ or $(z,x) \in E(H)$. Since the two cases are analogous, assume without the loss of generality that $(x,z) \in E(H)$.  Observe that $v \in \var(c)$ and $v \in \var(v)$; thus, $v \in \var(x) \cap \var(z)$. Since $v \in U$ it holds that $\lambda$ satisfies $(x,z)$; therefore, by \Cref{def:CSPInstance} it holds that $\lambda(x)_v = \lambda(z)_v$. Thus,
				$$s(v) = \lambda(x)_v = \lambda(z)_v = \lambda(y)_v.$$
				The first equality follows from \Cref{claim:auxc2} since $v \in U$. The last equality holds by \Cref{claim:auxc1} since $v \in U$, $y,z \in \psi(c)$, and $c \in U$. %The second equality holds since $v \in U$ and $x,z \in \psi(v)$
				%follows from \Cref{claim:auxc1} since $v \in U \cap \var(c) \cap \var(v)$ and since $()$ 
		\end{itemize}
		By the above, $s$ satisfies $c$ and the proof of the claim follows. 
	\end{claimproof}
	
	By \Cref{claim:satisfiedTildeC}, %instead of giving a lower bound on $\SAT(\phi)$ 
	it suffices to give a lower bound on $\left|\tilde{C}\right|$.
		Let $Q = V(G_{\phi}) \setminus U$ be the set of  all variables or clauses assigned to vertices in $H$ that participate in at least one unsatisfied constraint.  We first give an upper bound on the cardinality of $Q$. 
		
			\begin{claim}
			\label{claim:Qcar}
			$|Q| \leq \frac{ \left(1-\alpha\right) \cdot m}{\rho}$. 
		\end{claim}
		\begin{claimproof}
			%Since there are at most $\eps \cdot |E(H)|$ unsatisfied constraints, and each constraints corresponds to two vertices $x,y \in V(H)$ the number of literals assigned to vertices that participate in an unsatisfied constraint is bounded by 
			For every $\ell \in Q$ there is $e_{\ell} = (x_{\ell},y_{\ell}) \in E(H)$ such that (i) $\left\{x_{\ell},y_{\ell}\right\} \cap \psi(\ell) \neq \emptyset$ and (ii) it holds that $\left(\lambda(x_{\ell}),\lambda(y_{\ell})\right) \notin X_{e_{\ell}}$.  Define $F = \{e_{\ell} \mid \ell \in Q\}$. For all $e = (x,y) \in E(H)$ it holds that 
			\begin{equation}
				\label{eq:Fineq}
				\left|  \left\{    \ell \in Q \mid  e_{\ell} = e %\textnormal{ or } y_{\ell} = x
				\right\}\right| \leq \left|V_x(\psi) \cup V_{y}(\psi)\right| \leq \left|V_x(\psi)\right|+\left|V_y(\psi)\right| \leq 2 \cdot \Delta(\psi). %\leq |V_x(\psi)| \leq \Delta(\psi). 
			\end{equation} The first inequality holds since for every $\ell \in Q$ such that $e_{\ell} = e$ it holds that $\ell \in V_x(\psi)$ or $\ell \in V_y(\psi)$ implying that $\ell \in V_x(\psi) \cup V_y(\psi)$. The last inequality follows from the definition of $\Delta(\psi)$. %it holds that $$
			 Thus, 
			\begin{equation*}
				\label{eq:Qq}
				\begin{aligned}
					|Q| ={} & \sum_{e = (x,y) \in E(H) \textnormal{ s.t. } \left(\lambda(x),\lambda(y)\right) \notin X_{e}}		\left|  \left\{    \ell \in Q \mid  e_{\ell} = e 
					\right\}\right| 		
					\\\leq{} & 		\sum_{e = (x,y) \in E(H) \textnormal{ s.t. } \left(\lambda(x),\lambda(y)\right) \notin X_{e}}	2 \cdot \Delta(\psi)
					\\={} & 2 \cdot \left|\left\{ e = (x,y) \in E(H) \mid \left(\lambda(x),\lambda(y)\right) \notin X_{e} \right\}\right| \cdot \Delta(\psi)
						\\\leq{} & 2 \cdot \frac{\chi}{\log(k)} \cdot |E(H)| \cdot \Delta(\psi) 
							\\\leq{} & 2 \cdot \frac{\chi}{\log(k)} \cdot |E(H)| \cdot 
						Z \cdot \left(1+\frac{|V(G_{\phi})|+|E(G_{\phi})|}{k}\right) \cdot \log(k)
							\\\leq{} & 2 \cdot \chi \cdot 3 \cdot k \cdot 
						Z \cdot \left(1+\frac{n+m+3 \cdot m}{k}\right)
							\\\leq{} & 6 \cdot \chi \cdot k \cdot 
						Z \cdot \frac{\left(2 \cdot n+4 \cdot \rho \cdot n\right)}{k}
							\\={} & \chi \cdot 6 \cdot 
						Z \cdot \left(2+4 \cdot \rho\right) \cdot n
						\\\leq{} & \chi \cdot 6 \cdot 
						Z \cdot \left(2+4 \cdot \rho\right) \cdot \frac{m}{\tau}
						\\={} &\frac{ \left(1-\alpha\right) \cdot m}{\rho}.  
				\end{aligned}
			\end{equation*} The first equality holds since for every $\ell \in Q$ there is exactly one $e \in E(H)$ such that $\left(\lambda(x),\lambda(y)\right) \notin X_{e}$ and $e_{\ell} = e$. The first inequality follows from \eqref{eq:Fineq}. The second inequality uses the lower bound on the number of satisfied edges by $\lambda$. The third inequality follows from the depth guarantee of $\psi$ by \Cref{lem:embedding}. The fourth inequality holds since $|V(H)| \leq k$ by \Cref{lem:embedding}; additionally, since $H$ is $3$-regular it also implies that $|E(H)| \leq 3 \cdot k$. The fifth inequality holds since $k \leq n$ and since $m \leq \rho \cdot n$. The last equality follows from the selection of $\chi$ in \eqref{eq:chi}. By the above, the proof follows. 
		\end{claimproof}
	 
	 Hence, using \Cref{claim:Qcar},
	 \begin{equation}
	 	\label{eq:SATfin}
	 	\begin{aligned}
	 		\SAT(\phi) \geq{} & \left|\left\{   c \in C \mid  \textnormal{$s$ satisfies $c$}  \right\}\right|
	 		\\\geq{} & \left|\tilde{C}\right|
	 			\\={} & |C|- \left| \left\{   c \in C \mid c \notin U \textnormal{ or } \var(c) \not \subseteq U \right\}\right|
	 				\\\geq{} & |C|- |C \setminus U|- \sum_{c \in C \cap U}     |\var(c) \setminus U|   
	 					\\\geq{} & |C|- |C \setminus U|- \sum_{c \in C}     |\var(c) \setminus U|   
	 						\\={} & |C|- |C \setminus U|- \sum_{v \in V \cap Q } \left| \left\{   c \in C \mid v \in \var(c)  \right\}\right|   
	 				\\\geq{} & m - |Q| \cdot \rho
	 					\\\geq{} & m - (1-\alpha) \cdot m
	 						\\={} &  \alpha \cdot m. 
	 	\end{aligned}
	 \end{equation} The first inequality holds since $s$ is an assignment for $\phi$. The second inequality follows from \Cref{claim:satisfiedTildeC}. The first equality holds by \eqref{eq:Ctild}. The second equality follows by changing the order of summation. The fifth inequality holds since each variable appears in at most $\rho$ clauses; thus, for each $v \in V \cap Q$ there are at most $\rho$ clauses $c \in C$ such that $v \in \var(c)$.  The last inequality holds by \Cref{claim:Qcar}. By \eqref{eq:SATfin} the proof of the lemma follows. 
\end{proof}

In the following, we give an upper bound on the encoding size of reduced instances. Define a parameter $\mu = 20 \cdot Z \cdot L \cdot \rho$. We use the following auxiliary results. 

	\begin{lemma}
	\label{lem:varxBound}
		Let $\phi = (V,C)$   be a $(\tau,\rho)$\textnormal{-3-SAT} instance 
	on $n$ variables and $m$ clauses and let $k>6$ such that $k \leq \frac{n}{\log(n)}$, and let $(H,\psi) \leftarrow \textnormal{\textsf{Embedding}}(G_{\phi},k)$. Then, for all $x \in V(H)$ it holds that  $$\left|\{0,1\}^{\var(x)}\right| \leq 2^{6 \cdot Z   \cdot \rho \cdot \frac{n}{k}  \cdot \log(k)}.$$
\end{lemma}

\begin{proof}
	It holds that 
		\begin{equation*}
		\label{eq:SigmaBound}
		\begin{aligned}
			\left|\{0,1\}^{\var(x)}\right|
			\leq{} & \left|\{0,1\}^{3 \cdot |V_x(\psi)|}\right|
			\\\leq{} & \left|\{0,1\}^{3 \cdot \Delta\left(\psi\right)}\right|
			\\\leq{} &  2^{Z \cdot \left(1+\frac{|V(G_{\phi})|+|E(G_{\phi})|}{k}\right) \cdot \log(k)}
			\\\leq{} & 2^{Z \cdot \left(1+\frac{n+m+3 \cdot m}{k}\right) \cdot \log(k)}
			\\\leq{} &  2^{Z \cdot \left( \frac{2 \cdot n+4 \cdot \rho \cdot n}{k} \right) \cdot \log(k)}
			\\={} &  2^{Z \cdot \left(2+4 \cdot \rho\right) \cdot \frac{n}{k}  \cdot \log(k)}.
			\\\leq{} &  2^{6 \cdot Z   \cdot \rho \cdot \frac{n}{k}  \cdot \log(k)}.
		\end{aligned}
	\end{equation*}
	The first inequality holds since $|\var(\ell)| \leq 3$ for every $\ell \in V_x(\psi)$. The third inequality follows from the depth guarantee of $\psi$ using \Cref{lem:embedding}. The fifth inequality holds since $k \leq n$ and since $m \leq \rho \cdot n$.
\end{proof}

Using the above lemma, we can analyze the encoding size of reduced instances. 

	\begin{lemma}
	\label{lem:EncodingG}
	Let $\phi = (V,C)$   be a $(\tau,\rho)$\textnormal{-3-SAT} instance 
	on $n$ variables and $m$ clauses and let $k>6$ such that $k \leq \frac{n}{\log(n)}$. Then, $|\Gamma(\phi,k)| \leq 	2^{\mu \cdot \frac{n}{k}  \cdot \log(k)}$.
\end{lemma}
\begin{proof}
%	By \Cref{lem:varxBound}, for all $x \in V(H)$ it holds that 
%	\begin{equation}
%		\label{eq:SigmaBound}
%		\begin{aligned}
%			\left|\Sigma_x\right| \leq \left|\{0,1\}^{\var(x)}\right|
%			 \leq   2^{6 \cdot Z   \cdot \rho \cdot \frac{n}{k}  \cdot \log(k)}.
%		\end{aligned}
%	\end{equation}
	%The second inequality holds since $|\var(\ell)| \leq 3$ for every $\ell \in V_x(\psi)$. The fourth inequality follows from the depth guarantee of $\psi$ using \Cref{lem:embedding}. The sixth inequality holds since $k \leq n$ and since $m \leq \rho \cdot n$. 
	%By \eqref{eq:SigmaBound} 
	Observe that the size of the alphabet of $\Gamma(\phi,k)$ can be bounded by:
%	\begin{equation}
%		\label{eq:SigmaBound2}
%		\begin{aligned}
%			|\Sigma| \leq \sum_{x \in V(H)} \left|\Sigma_x\right|
%			\leq k \cdot 2^{6 \cdot Z   \cdot \rho \cdot \frac{n}{k}  \cdot \log(k)}.
%			%	\\\leq{} & 2^k \cdot 10^{\frac{n}{k} \cdot \log(k)} 
%			%	\\={} & 2^k \cdot 2^{4 \cdot \frac{n}{k} \cdot \log(k)}
%		\end{aligned}
%	\end{equation}
	\begin{equation}
	\label{eq:SigmaBound2}
	\begin{aligned}
		|\Sigma| = \abs{\bigcup_{x \in V(H)} \{0,1\}^{\var(x)}} \leq \sum_{x \in V(H)} \left|\{0,1\}^{\var(x)}\right|
		\leq \abs{V(H)} \cdot 2^{6 \cdot Z   \cdot \rho \cdot \frac{n}{k}  \cdot \log(k)} \leq k \cdot 2^{6 \cdot Z   \cdot \rho \cdot \frac{n}{k}  \cdot \log(k)}.
	\end{aligned}
\end{equation} The second inequality follows from \Cref{lem:varxBound}. The last inequality holds since $\abs{V(H)} \leq k$ by \Cref{lem:embedding}. 
	%	\\\leq{} & \eps \cdot 6 \cdot k \cdot Z \cdot \left(1+\frac{2n+m+3 \cdot m+n}{k}\right) \cdot \log(k)
	%\\\leq{} & \eps \cdot 6 \cdot k \cdot Z \cdot \left( \frac{6n+8 \cdot m}{k} \right)\cdot \log(k)
	The encoding size of $H$, that is $|H|$, can be bounded by the number of vertices and edges in $H$:\footnote{For simplicity, we do not consider the encoding size of each vertex/edge but only their number.}
	\begin{equation}
		\label{eq:EncodingH}
		|H| \leq \left|V(H)\right|+\left|E(H)\right| \leq k+3 \cdot k = 4 \cdot k.
	\end{equation}
	The second inequality holds since $\abs{V(H)} \leq k$ and since the graph $H$ obtained from $\textnormal{\textsf{Embedding}}(G_{\phi},k)$ is $3$-regular by \Cref{lem:embedding}; thus, it holds that $\abs{E(H)} \leq 3 \cdot k$. Finally, the encoding size of $X$, can be bounded by 
	\begin{equation}
		\label{eq:EncodingX}
		\begin{aligned}
			\sum_{(x,y) \in E(H)} \left|X_{(x,y)}\right| \leq{} & 	\sum_{(x,y) \in E(H)} \left|\Sigma_x\right| \cdot \left|\Sigma_y\right| 
			\\\leq{} & |E(H)| \cdot \left(2^{6 \cdot Z   \cdot \rho \cdot \frac{n}{k}  \cdot \log(k)}\right)^2 %2^{Z \cdot \left(2+4 \cdot \rho\right) \cdot \frac{n}{k}  \cdot \log(k)} \cdot 2^{Z \cdot \left(2+4 \cdot \rho\right) \cdot \frac{n}{k}  \cdot \log(k)}
			\\\leq{} & 3 \cdot k \cdot 2^{12 \cdot Z   \cdot \rho \cdot \frac{n}{k}  \cdot \log(k)}.
		\end{aligned}
	\end{equation} The second inequality follows from \Cref{lem:varxBound}. The last inequality holds since $H$ is $3$-regular and $|V(H)| \leq k$ by \Cref{lem:embedding}.  Therefore, by \eqref{eq:SigmaBound2}, \eqref{eq:EncodingH}, and \eqref{eq:EncodingX} the encoding size of $\Gamma(\phi,k)$ can be bounded~by 
	\begin{equation*}
		\label{eq:sB2}
		\begin{aligned}
			|\Gamma(\phi,k)| \leq{} & |H|+|\Sigma|+	\sum_{(x,y) \in E(H)} \left|X_{(x,y)}\right|  
			\\\leq{} & 4 \cdot k+ k \cdot 2^{Z \cdot 6 \cdot \rho \cdot \frac{n}{k}  \cdot \log(k)}+3 \cdot k \cdot 2^{12 \cdot Z \cdot \rho \cdot \frac{n}{k}  \cdot \log(k)}
			\\\leq{} &
			8 \cdot k \cdot 2^{12 \cdot Z \cdot \rho \cdot \frac{n}{k}  \cdot \log(k)}
			\\\leq{} &
			2^{8 \cdot \log(k)} \cdot 2^{12 \cdot Z \cdot \rho \cdot \frac{n}{k}  \cdot \log(k)}
		%	\\\leq{} &
			%2^{3 \cdot Z \cdot \left(2+4 \cdot \rho\right) \cdot \frac{n}{k}  \cdot \log(k)}
			\\\leq{} &
			2^{20 \cdot Z \cdot \rho \cdot \frac{n}{k}  \cdot \log(k)}
				\\\leq{} &
			2^{\mu \cdot \frac{n}{k}  \cdot \log(k)}. 
		\end{aligned}
	\end{equation*} The fifth inequality holds since $k \leq n$ and $\rho,Z \geq 1$; thus, $8 \cdot \log(k) \leq 8 \cdot Z \cdot \rho \cdot \frac{n}{k} \cdot \log(k)$, implying the inequality. The last inequality follows from the selection of $\mu$. By the above, the proof follows. %The above equation implies the statement of the lemma. 
\end{proof}

Using the bound on the encoding size of reduced instances, we can obtain an upper bound on the running time of the reduction. 



	\begin{lemma}
	\label{lem:Grunningtime}
		Let $\phi = (V,C)$   be a $(\tau,\rho)$\textnormal{-3-SAT} instance 
	on $n$ variables and $m$ clauses and let $k>6$ such that $k \leq \frac{n}{\log (n)}$. Then, $\Gamma(\phi,k)$ can be computed from $\phi$ and $k$ in time $O \left(2^{\mu \cdot \frac{n}{k}  \cdot \log(k)} \right)$.
\end{lemma}

\begin{proof}
	By \Cref{def:CSPInstance}, the instance $\Gamma(\phi,k)$ can be computed as follows. 
	\begin{enumerate}
		\item Execute Algorithm \textnormal{\textsf{Embedding}} on input $G_{\phi}$ and $k$ and obtain the graph $H$ and the connected embedding $\psi$. \label{time:1}
		\item %For every $x \in V(H)$ compute $\Sigma_{x}$ and construct 
		Compute $\Sigma = \bigcup_{x \in V(H)}  \{0,1\}^{\var(x)}$ directly. \label{time:2}
		\item For every $x \in V(H)$ compute $\Sigma_{x}$.
			\item For every $(x,y) \in E(H)$ compute $X_{(x,y)}$ and construct $X = \left\{X_{(x,y)}\right\}_{(x,y) \in E(H)}$.\label{time:3}
	\end{enumerate}

	
	We analyze below the running time of the above steps.
	
	\begin{enumerate}
		\item By \Cref{lem:embedding} it holds that Algorithm \textnormal{\textsf{Embedding}} on input $G_{\phi}$ and $k$ can be computed in time 
		\begin{equation}
			\label{eq:CompG1}
			\begin{aligned}
				\left(|V(G_{\phi})|+|E(G_{\phi})|\right)^{L} \leq{} &
				\left(n+m+3 \cdot m\right)^L
				\\\leq{} &
				\left(n+4 \cdot \rho \cdot n\right)^L
				\\\leq{} &
				\left(5 \cdot \rho \cdot n\right)^L
				\\\leq{} &
				2^{ \log \left(5 \cdot \rho \cdot n \right) \cdot L}
				\\\leq{} &
				2^{ 5 \cdot \rho \cdot  L \cdot \log \left( n\right) }
				\\\leq{} &
				2^{ 5 \cdot \rho \cdot  L \cdot \frac{n}{k} \cdot \log(k)} 
			\end{aligned}
		\end{equation}
		The sixth inequality holds since $k \leq \frac{n}{\log(n)}$.
		
		\item  It holds that $\Sigma$ can be computed naively in time $|V(H)| \cdot \abs{\max_{x \in V(H)} \var(x)} \leq k \cdot 2^{6 \cdot Z   \cdot \rho \cdot \frac{n}{k}  \cdot \log(k)}$. The inequality holds since there are at most $k$ vertices in $H$ by \Cref{lem:embedding} and in addition by \Cref{lem:varxBound}.  
		
		\item For every  $x \in V(H)$ it holds that $\Sigma_x$ can be computed naively in time $\abs{\{0,1\}^{\var(x)}}$; thus, $\Sigma_x$ can be computed in time bounded by $2^{6 \cdot Z   \cdot \rho \cdot \frac{n}{k}  \cdot \log(k)}$ using \Cref{lem:varxBound}.
		
		\item For every  $(x,y) \in E(H)$ it holds that $X_{(x,y)}$ can be computed naively in time $\abs{\{0,1\}^{\var(x)} \times \{0,1\}^{\var(y)}}$. Thus, $X_{(x,y)}$ can be computed in time bounded by $\left(2^{6 \cdot Z   \cdot \rho \cdot \frac{n}{k}  \cdot \log(k)}\right)^2 = 2^{12 \cdot Z   \cdot \rho \cdot \frac{n}{k}  \cdot \log(k)}$ using \Cref{lem:varxBound}. Therefore, $X$ can be computed in time $|E(H)| \cdot 2^{6 \cdot Z   \cdot \rho \cdot \frac{n}{k}  \cdot \log(k)} \leq 3 \cdot k \cdot 2^{6 \cdot Z   \cdot \rho \cdot \frac{n}{k}  \cdot \log(k)}$. he inequality holds since there are at most $k$ vertices in $H$ and since $H$ is $3$-regular by \Cref{lem:embedding}; hence $|E(H)| \leq 3 \cdot k$. 
	\end{enumerate}
	  %In addition, 
	
	 By the above, $\Gamma(\phi,k)$ can be computed from $\phi$ and $k$ in time 
%	\begin{equation}
%		\label{eq:CompG}
%		\begin{aligned}
%			|\Gamma(\phi,k)|+\left(|V(G_{\phi})|+|E(G_{\phi})|\right)^{L} \leq{} &
%		2^{18 \cdot Z \cdot \rho \cdot \frac{n}{k}  \cdot \log(k)}+\left(n+m+3 \cdot m\right)^L
%			\\\leq{} &
%				2^{18 \cdot Z \cdot \rho \cdot \frac{n}{k}  \cdot \log(k)}+\left(n+4 \cdot \rho \cdot n\right)^L
%			%2^{16 \cdot Z \cdot \left(6+8 \cdot \rho\right) \cdot \frac{n}{k}  \cdot \log(k)}+\left(2\cdot n+\rho \cdot n+3 \cdot \rho \cdot n+n\right)^L
%			\\\leq{} &
%				2^{18 \cdot Z \cdot \rho \cdot \frac{n}{k}  \cdot \log(k)}+\left(5 \cdot \rho \cdot n\right)^L
%			%2^{16 \cdot Z \cdot \left(6+8 \cdot \rho\right) \cdot \frac{n}{k}  \cdot \log(k)}+\left(3 \cdot n+4 \cdot \rho \cdot n\right)^L
%			\\\leq{} &
%			2^{18 \cdot Z \cdot \rho \cdot \frac{n}{k}  \cdot \log(k)}+2^{ \log \left(5 \cdot \rho \cdot n \right) \cdot L}
%				\\\leq{} &
%			2^{18 \cdot Z \cdot \rho \cdot \frac{n}{k}  \cdot \log(k)}+2^{ 5 \cdot \rho \cdot  L \cdot \log \left( n\right) }
%				\\\leq{} &
%			2^{18 \cdot Z \cdot \rho \cdot \frac{n}{k}  \cdot \log(k)}+2^{ 5 \cdot \rho \cdot  L \cdot \frac{n}{k}} 
%				\\\leq{} &
%			2^{18 \cdot Z \cdot \rho \cdot \frac{n}{k}  \cdot \log(k)} \cdot 2^{ 5 \cdot \rho \cdot  L \cdot \frac{n}{k}} 
%				\\\leq{} &
%			2^{20 \cdot L \cdot Z \cdot \rho \cdot \frac{n}{k}  \cdot \log(k)}. 
%			\\={} &
%			2^{\mu \cdot \frac{n}{k}  \cdot \log(k)}. 
%		%	2^{16 \cdot Z \cdot \left(6+8 \cdot \rho\right) \cdot \frac{n}{k}  \cdot \log(k)}+2^{\left(3+4 \cdot \rho\right) \cdot L \cdot \log (n)}
%		%	\\\leq{} &
%%			2^{16 \cdot Z \cdot \left(6+8 \cdot \rho\right) \cdot \frac{n}{k}  \cdot \log(k)}+2^{\left(3+4 \cdot \rho\right) \cdot L \cdot \frac{n}{k}}
%%			\\\leq{} &
%%			2^{17 \cdot Z \cdot L \cdot \left(6+8 \cdot \rho\right) \cdot \frac{n}{k}  \cdot \log(k)}
%		\end{aligned}
%	\end{equation} The first inequality holds by \Cref{lem:EncodingG}. The second inequality holds since $m \leq \rho \cdot n$. 
\begin{equation}
	\label{eq:AQQQ}
	\begin{aligned}
	O \left(2^{ 5 \cdot \rho \cdot  L \cdot \frac{n}{k} \cdot \log(k)} +2 \cdot k \cdot 2^{6 \cdot Z   \cdot \rho \cdot \frac{n}{k}  \cdot \log(k)}+ 3 \cdot k \cdot 2^{6 \cdot Z   \cdot \rho \cdot \frac{n}{k}  \cdot \log(k)}\right) \leq{} & O \left( k \cdot 2^{6 \cdot Z  \cdot L \cdot \rho \cdot \frac{n}{k}  \cdot \log(k)}\right)
	\\={} &
	O \left( 2^{\log(k)+6 \cdot Z  \cdot L \cdot \rho \cdot \frac{n}{k}  \cdot \log(k)}\right)
		\\\leq{} &
	O \left( 2^{7 \cdot Z  \cdot L \cdot \rho \cdot \frac{n}{k}  \cdot \log(k)}\right)
	\\\leq{} &
	O \left( 2^{\mu \cdot \frac{n}{k}  \cdot \log(k)}\right). 
	\end{aligned}
\end{equation} The second inequality holds since $Z  \cdot L \cdot \rho \cdot \frac{n}{k} \geq 1$. The (last) equality follows from the selection of~$\mu$. The proof follows from \eqref{eq:AQQQ}. 
\end{proof}

We can finally prove \Cref{thm:SATtoCSP}. 

\subsubsection*{Proof of \Cref{thm:SATtoCSP}:} 
Let $\phi = (V,C)$   be a $(\tau,\rho)$\textnormal{-3-SAT} instance 
on $n$ variables and $m$ clauses and let $k>6$ such that $k \leq \frac{n}{\log(n)}$. Then, the running time guarantee follows from \Cref{lem:Grunningtime}. In addition, the two directions of the reduction, written in \Cref{prop:c1,prop:c2}, follow from \Cref{lem:CSPeasy} and \Cref{lem:CSPhard}, respectively. Moreover, the bound on the encoding size of $\Gamma(\phi,k)$ (see \Cref{prop:c3})  follows from \Cref{lem:EncodingG}. Finally, \Cref{prop:c4} follows from \Cref{lem:embedding}. \qed
%By \Cref{def:CSPInstance} and \Cref{label}
%OLD VERSION!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!





































\comment{



















\begin{proof}
	Let $\tau,\rho,\delta$, and $\alpha$ be the constants described in \Cref{thm:GAP-eth}. Fix some $n \in \mathbb{N}$ and fix a 3-SAT formula $\phi = (V,C)$ with $n = |V|$ variables and $m = |C|$ clauses such that $m \leq \rho \cdot n$ and that for every $v \in V$ there are at most $\rho$ clauses $c \in C$ such that $v$ or $\overline{v}$ appear in $c$. Note that $\phi$ satisfies the conditions of the 3-SAT instances described in \Cref{thm:GAP-eth}. Let $k>6$ such that $k \leq \frac{n}{\log (n)}$. Define a graph $G = (V(G,E(G)))$ such that $V(G) = V \cup \overline{V} \cup C$ and edges are between (i) every literal (a variable or a negation of a variable) to a clause in which the literal participates and (ii) there is an edge between every variable to its negation: $$E(G) = \{(a,c) \in \left(V \cup \overline{V}\right) \times C~|~ a \in c\} \cup \{(v,\overline{v})~|~v \in V\}.$$
	
	As each clause is an endpoint of at most three edges in $G$, and there are only $n$ edges in $G$ without a clause endpoint, we have the following observation. %(a variable or its negation) appears in at most 
	\begin{obs}
		$|V(G)| \leq 2 \cdot n+m$ and $|E(G)| \leq 3 \cdot m+n$. 
	\end{obs}
	
	Let $(H,\psi) = \cA(G,k)$ be the 3-regular graph $H$ and the connected embedding $\psi : V(G) \rightarrow 2^{V(H)}$ of $G$ to $H$ obtained by applying the algorithm $\cA$ described in \Cref{lem:embedding} on input $G$ and $k$. %Define $H$ by adding to $H'$ all loops $\{(x,x)~|~x \in V(H)$, 
	%We define a 2-CSP instance $\Gamma = (H,\Sigma,X)$ as follows, with the graph $H$ described above. 
	For every $x \in V(H)$ we define an alphabet $\Sigma_x$ containing assignments to vertices $v \in V(G)$ that are mapped to a subgraph $\psi(v)$ containing $x$. 
	
	\begin{definition}
		\label{def:Sigma_x}
		For every $x \in V(H)$ define $\Sigma_x$ as the set of all vectors $\by \in \left(\{0,1\} \cup \{0,1\}^3  \right)^{V_x(\psi)}$ that satisfy the following properties. 
		\begin{enumerate}
			\item For every $\ell \in V_x(\psi) \cap \left(V \cup \overline{V}\right)$ it holds that $\by_{\ell} \in \{0,1\}$. \label{prop:a1}
				\item For every $c \in V_x(\psi) \cap C$ it holds that $\by_{c} \in \{0,1\}^3$.\label{prop:a2}
				\item For every $v \in V(G)$ such that $v \in V_x(\psi)$ and $\overline{v} \in V_x(\psi)$ it holds that $\by_v = 1-\by_{\overline{v}}$.  \label{prop:a3}
				\item For all $c \in C$ and $i \in [3]$ such that $ \overline{c}[i],c \in V_x(\psi)$ it holds that  $\by_{\overline{c}[i]} = 1-\by_{c}[i]$.\label{prop:a4}
				\item For all $c \in C$ and $i \in [3]$ such that $c[i],c \in V_x(\psi)$ it holds that $\by_{c[i]} = \by_{c}[i]$. \label{prop:a5}
				\item For every $c \in C \cap V_x(\psi)$ it holds that $\by_{c}[1]+\by_{c}[2]+\by_{c}[3] \geq 1$. \label{prop:a6}
		\end{enumerate} 
	\end{definition}
	
%	in phases as follows. Define $\Sigma^1_x = \left(\{0,1\} \cup \{0,1\}^3  \right)^{V_x(\psi)}$ as all 0/1-assignments to all vertices $v \in V(G)$ that are mapped to a subgraph $\psi(v)$ containing $x$. Now, define 
	%$$\Sigma^2_x = \left\{ \by \in \Sigma^1_x ~\big|~ \by_{\ell} \in \{0,1\} ~\forall \ell \in V_x(\psi) \cap \left(V \cup \overline{V}\right)  \right\}$$  
	%$$\Sigma^3_x = \left\{ \by \in \Sigma^1_x ~\big|~ \by_{c} \in \{0,1\}^3 ~\forall c \in V_x(\psi) \cap C  \right\}$$  
%	Define $\Sigma^4_x = \Sigma^2_x \cap \Sigma^3_x$ and define 
	%$$\Sigma^5_x = \left\{ \by \in \Sigma^4_x ~\big|~ \by_v = 1-\by_{\overline{v}} ~\forall v \in V(G) \text{ s.t. } v,\overline{v} \in V_x(\psi)  \right\}$$ 
	%Define
	%$$\Sigma^6_x = \left\{ \by \in \Sigma^5_x ~\big|~ \by_{c[i]} = \by_{c}[i] ~\forall c \in C, i \in [3] \text{ s.t. } c[i],c \in V_x(\psi) \right\}$$ 
	%$$\Sigma^7_x = \left\{ \by \in \Sigma^6_x ~\big|~ \by_{\overline{c}[i]} = 1-\by_{c}[i] ~\forall c \in C, i \in [3] \text{ s.t. } \overline{c}[i],c \in V_x(\psi) \right\}$$ 
%	and finally define 
%	$$\Sigma_x = \left\{ \by \in \Sigma^7_x ~\big|~ \by_{c}[1]+\by_{c}[2]+\by_{c}[3] \geq 1 ~\forall c \in C \cap V_x(\psi) \right\}$$ 
	%= 1-\by_{\overline{v}} ~\forall v \in V(G) \text{ s.t. } v,\overline{v} \in V_x(\psi)
	
	%	$$\Sigma^2_x = \left\{ \by \in \Sigma^1_x ~\big|~ \left(\by_v = 1-\by_{\overline{v}}\forall v \in V(G) \right) \textnormal{ and }   \left(\by_a = 1 \forall (a,c) \in E(G) \text{ s.t. } a,c \in V_x(\psi) \right) \right\}$$  
	
	We define below all  {\em consistent} pairs $(\bx,\by) \in \Sigma_x \times \Sigma_{y}$ for every edge $(x,y) \in E(H)$. 
		\begin{definition}
		\label{def:Xxy}
		For every $(x,y) \in E(H)$ define $X_{(x,y)}$ as the set of all {\em consistent} pairs $(\bx,\by) \in \Sigma_x \times \Sigma_{y}$ that satisfy the following properties. 
		\begin{enumerate}
			\item For every $\ell \in V_x(\psi) \cap \left(V \cup \overline{V}\right)$ such that $\overline{\ell} \in V_y(\psi)$ it holds that $\bx_{\ell} = 1-\by_{\overline{\ell}}$. \label{prop:b1}
				\item For every $\ell \in V_x(\psi) \cap V_y(\psi)$ it holds that $\bx_{\ell} = \by_{\ell}$. \label{prop:b2}
					\item For all $c \in C$ and $i \in [3]$ such that $c[i] \in V_x(\psi)$ and $c \in V_y(\psi)$ it holds that $ \bx_{c[i]} = \by_{c}[i]$. \label{prop:b3}
						\item For all $c \in C$ and $i \in [3]$ such that $c \in V_x(\psi)$ and $c[i] \in V_y(\psi)$ it holds that $ \bx_{c}[i] = \by_{c[i]}$.  \label{prop:b4}
		\end{enumerate} 
	\end{definition}
	
	
	 %For every $(a,b) \in E(H)$ define the constraints 
	 %$$X^1_{(x,y)} = \{ (\bx,\by) \in \Sigma_x \times \Sigma_{y}~|~  \bx_v = 1-\by_{\overline{v}} ~\forall v \in V \text{ s.t. } v \in  V_x(\psi) \textnormal{ and } \overline{v} \in  V_y(\psi)\}$$
	%$$X^2_{(x,y)} = \{ (\bx,\by) \in \Sigma_x \times \Sigma_{y}~|~  \overline{x}_{\overline{v}} = 1-\by_{v} ~\forall v \in V \text{ s.t. } \overline{v} \in  V_x(\psi) \textnormal{ and } v \in  V_y(\psi)\}$$
	%$$X^3_{(x,y)} = \{ (\bx,\by) \in \Sigma_x \times \Sigma_{y}~|~  \bx_v = \by_{v} ~\forall v \in V \text{ s.t. } v \in  V_x(\psi) \cap V_y(\psi)\}$$
	%$$X^4_{(x,y)} = \{ (\bx,\by) \in \Sigma_x \times \Sigma_{y}~|~  \bx_{\overline{v}} = \by_{\overline{v}} ~\forall v \in V \text{ s.t. } \overline{v} \in  V_x(\psi) \cap V_y(\psi)\}$$
	%$$X^5_{(x,y)} = \{ (\bx,\by) \in \Sigma_x \times \Sigma_{y}~|~  \bx_{c[i]} = \by_{c}[i] ~\forall c \in C,i \in [3] \text{ s.t. } c[i] \in V_x(\psi), c \in V_y(\psi)\}$$
	%$$X^6_{(x,y)} = \{ (\bx,\by) \in \Sigma_x \times \Sigma_{y}~|~  \bx_{c}[i] = \by_{c[i]} ~\forall c \in C,i \in [3] \text{ s.t. } c \in V_x(\psi), c[i] \in V_y(\psi)\}$$
	%$$X^7_{(x,y)} = \{ (\bx,\by) \in \Sigma_x \times \Sigma_{y}~|~  \bx_{c} = \by_{c} ~\forall c \in C \cap V_x(\psi) \cap V_y(\psi)\}$$
	%and finally define $X_{(x,y)} = \bigcup_{j \in [7]} X^j_{xy}$. 
	
	
	We define a 2-CSP instance $\Gamma = (H,\Sigma,X)$ with the graph $H$ obtained from the embedding, the alphabet $\Sigma = \bigcup_{x \in V(H)} \Sigma_x$, and constraints $X = \left\{ X_{(x,y)}\right\}_{(x,y) \in E(H)}$.
	We prove the properties of the reduction below. 

	\begin{claim}
		\label{claim:completeCSP}
		If $\SAT(\phi) = m$ then $\CSP(\Gamma) = |E(H)|$. 
	\end{claim}
	\begin{claimproof}
		Let $s: V\rightarrow \{0,1\}$ be a satisfying assignment of $\phi$. With a slight abuse of notation, for a negation of variable $\overline{v} \in \overline{V}$ define $s(\overline{v}) = 1-s(v)$. Define an assignment $\sigma: V(H) \rightarrow \Sigma$ for $\Gamma$ such that for every $x \in V(H)$ define $\sigma(x)$ as follows. For $\ell \in V_x(\psi)$ define the $\ell$-th entry of $\sigma(x)$, that is $\sigma(x)_{\ell}$, as:
		\begin{equation}
			\label{eq:cases}
			\sigma(x)_{\ell} = \begin{cases}
				s(\ell), & \text{if } \ell \in \left(V\cup\overline{V}\right) \\
				%1-s(\ell), & \text{if } \ell \in \overline{V} \\
				\left(s(c[1]), s(c[2]),s(c[3])\right), & \text{if } \ell \in C
			\end{cases}
		\end{equation}
%		$$\sigma(x)_{\ell} = \begin{cases}
%			s(\ell), & \text{if } \ell \in \left(V\cup\overline{V}\right) \\
%			%1-s(\ell), & \text{if } \ell \in \overline{V} \\
%			\left(s(c[1]), s(c[2]),s(c[3])\right), & \text{if } \ell \in C
%		\end{cases}$$
		We prove that $\sigma$ satisfies all constraints of $\Gamma$. Consider some constraint $(x,y) \in E(H)$. We first show that $\sigma(x) \in \Sigma_x$ (and analogously $\sigma(y) \in \Sigma_y$). We prove that $\sigma(x)$ satisfies all properties of \Cref{def:Sigma_x}.
		\begin{enumerate}
			\item For every $\ell \in V_x(\psi) \cap \left(V \cup \overline{V}\right)$ it holds that $\sigma(x)_{\ell} \in \{0,1\}$ by \eqref{eq:cases}. 
		\item For every $c \in V_x(\psi) \cap C$ it holds that $\sigma(x)_{c} \in \{0,1\}^3$ by \eqref{eq:cases}. 
		\item For every $v \in V(G)$ such that $v \in V_x(\psi)$ and $\overline{v} \in V_x(\psi)$ it holds that $$\sigma(x)_v = s(v) = 1-s\left(\overline{v}\right) = 1-\sigma(x)_{\overline{v}}.$$ 
		\item For all $c \in C$ and $i \in [3]$ such that $ \overline{c}[i],c \in V_x(\psi)$ by \eqref{eq:cases} it holds that  $$\sigma(x)_{\overline{c}[i]} = s \left(\overline{c}[i]\right) = 1-s\left(c[i]\right) = 1-\sigma(x)_{c}[i] = 1-s \left(c[i]\right) = 1-\sigma(x)_{c}[i]$$
		\item For all $c \in C$ and $i \in [3]$ such that $c[i],c \in V_x(\psi)$ by \eqref{eq:cases} it holds that $\sigma(x)_{c[i]} = s \left(c[i]\right) = \sigma(x)_{c}[i]$. 
		\item For every $c \in C \cap V_x(\psi)$, since $s$ is a satisfying assignment for $\phi$ by \eqref{eq:cases} it holds that $$\sigma(x)_{c}[1]+\sigma(x)_{c}[2]+\sigma(x)_{c}[3] = s\left(c[1]\right)+ s\left(c[2]\right)+s\left(c[3]\right) \geq 1$$. 
		\end{enumerate} Thus, we conclude that $\sigma(x) \in \Sigma_x$ and analogously it holds that $\sigma(y) \in \Sigma_y$. it remains to show that $(\sigma(x),\sigma(y)) \in X_{(x,y)}$. We do so using the properties stated in \Cref{def:Xxy}. 
			\begin{enumerate}
			\item For every $\ell \in V_x(\psi) \cap \left(V \cup \overline{V}\right)$ such that $\overline{\ell} \in V_y(\psi)$ by \eqref{eq:cases} it holds that $$\sigma(x)_{\ell} = s(\ell) = 1-s \left(\overline{\ell}\right) = 1-\sigma(y)_{\overline{\ell}}.$$
			\item For every $\ell \in V_x(\psi) \cap V_y(\psi)$ by \eqref{eq:cases} it holds that $\sigma(x)_{\ell} = s(\ell) =  \sigma(y)_{\ell}$.  
			\item For all $c \in C$ and $i \in [3]$ such that $c[i] \in V_x(\psi)$ and $c \in V_y(\psi)$ by \eqref{eq:cases} it holds that $$\sigma(x)_{c[i]} = s \left(c[i]\right) = \sigma(y)_{c}[i].$$ 
			\item For all $c \in C$ and $i \in [3]$ such that $c \in V_x(\psi)$ and $c[i] \in V_y(\psi)$ by \eqref{eq:cases} it holds that $$ \sigma(x)_{c}[i] = s \left(c[i]\right)  =  \sigma(y)_{c[i]}.$$
		\end{enumerate} 
		Thus, $\sigma$ satisfies all constraints $(x,y) \in E(H)$. This implies  that $\CSP(\Gamma) = |E(H)|$.  
		%If $\ell$ It also holds that $\sigma(x)_{\ell}$
		%	where $\oplus$ denotes tuple concatenation. 
	\end{claimproof}
	
	
	Define an error margin parameter used in the following analysis as $$\eps = \frac{ (1-\alpha)}{\rho} \cdot \frac{1}{6 \cdot Z \cdot \left(\frac{6}{\tau}+8 \right) \cdot \log(k)}.$$  The selection of $\eps$ becomes clear in the following claim. Since $Z$ is a constant by \Cref{lem:embedding} and $\alpha,\rho,\tau$ are constants by \Cref{thm:GAP-eth} we remark that $\frac{1}{\eps} = \Theta \left(\log (k)\right)$. 
	
	\begin{claim}
		\label{claim:soundCSP}
		If $\CSP(\Gamma) \geq (1-\eps) \cdot |E(H)|$ then $\SAT(\phi) \geq \alpha \cdot m$.  
	\end{claim}
	\begin{claimproof}
		Let $\sigma: V(H) \rightarrow \Sigma$ be an assignment for $\Gamma$ that satisfies at least $(1-\eps) \cdot |E(H)|$ constraints. Define 
		$$U = \left\{\ell \in V(G)~|~\left(\sigma(x),\sigma(y)\right) \in X_{(x,y)} ~\forall (x,y) \in E(H) \textnormal{ s.t. }  x \in \psi(\ell) \textnormal{ or } y \in \psi(\ell)\right\}$$
		be all literals or clauses such that every vertex $v$ in their subgraph $\psi(\ell)$ and every constraint $(x,y) \in E(H)$, such that $v= x$ or $v = y$, is satisfied.  
		
		
		For all $u \in U$ choose some arbitrary $x \in \psi(u)$ and define $r(u) = x$; there is such $x$ since $\psi(u) \neq \emptyset$. 
		Define an assignment  $s: V\rightarrow \{0,1\}$  for $\phi$ by
		\begin{equation}
			\label{eq:ass1n}
		s(v) = \begin{cases}
		\sigma(r(v))_{v}, & \textnormal{if } v \in U \\
			0, & \textnormal{else }
		\end{cases}
		\end{equation} for all $v \in V$. For all $\overline{v} \in \overline{V}$ define $s\left(\overline{v}\right) = 1-s(v)$. 
		%such that for all $ u \in U \cap V$ define $s(u) = \sigma(r(u))_{u}$ (resp. define $s(u) = \sigma(r(u))_{u}$ for $u\in U \cap \overline{V}$) and for $v \in (V \cup \overline{V}) \setminus U$ define $s(v) \in \{0,1\}$ arbitrarily. 
		We first prove that for all $u \in U$ and all $y \in \psi(u)$ it holds that $s(u) = \sigma(y)_{u}$. Since $\psi$ is a connected embedding of $G$ in $H$ it holds that
		$\psi(u)$ is a connected subgraph of $H$; thus, there is a path from $r(u)$ to $y$ contained in $\psi(u)$. Let $r(u) = y_1, \ldots, y_t$ be such a path between $r(u)$ and $y$ in $\psi(u)$. Since $u \in U$ and by the definition of the constraints $X$ (see \Cref{def:Xxy}), for every $i \in [t-1]$
		it holds that $ \sigma(y_i)_{u} =  \sigma(y_{i+1})_{u}$. Therefore, for all $y \in \psi(u)$ it holds that $s(u) = \sigma(y)_{u}$. 
		
		Let $\tilde{C} = \left\{c \in C \cap U \mid c[i] \in U~\forall i \in [3] \right\}$ be the set of clauses in $U$ where all literals that appear in them are also in $U$. 
		We show that all clauses in $\tilde{C}$ are satisfied by $s$. Let $c \in \tilde{C}$. Then, % such that $c[i] \in U$ for all $i \in [3]$.  Then,
		\begin{equation*}
			\label{eq:sB2}
			\begin{aligned}
				s(c[1])+s(c[2])+s(c[3]) ={} & \sigma(r(c[1]))_{c[1]} +\sigma(r(c[2]))_{c[2]}+\sigma(r(c[3]))_{c[3]} \\
				={} &\sigma(r(c))_{c} [1]+\sigma(r(c))_{c} [2]+\sigma(r(c))_{c} [3] 
				\\  \geq{} & 1.
			\end{aligned}
		\end{equation*}
		The first equality follows from the definition of $s$ in \eqref{eq:ass1n}. %since $c \in C \cap U$; thus, it holds that $s(c[i]) = \sigma(r(c[i]))_{c[i]}$ as it is a constraint of $c$, and the equality follows from the definition of $\Sigma_{r(c)}$. 
		The second equality holds since $\psi$ is a connected embedding: thus, there is a constraint in $E(H)$ that requires that $\sigma(r(c))_{c} [i] = \sigma(r(c))_{c[i]} $ for all $i \in [3]$ since there are no isolated edges. %, either by a loop in $H$ or by a regular edge. 
		This constraint is satisfied since $c \in C \cap U$ and $c[i] \in U$ for all $i \in [3]$ as $c \in \tilde{C}$. The last inequality holds since all constraints involving $c$ are satisfied since $c \in U$, and the above is on of the conditions in the constraints (see the definition of $\Sigma_x$ in \Cref{def:Sigma_x}).   By the above, all clauses $c \in \tilde{C}$ are satisfied by $s$. Hence, to conclude, it suffices to give a lower bound on the cardinality of $\tilde{C}$. 
		
		
		Let $Q = V(G) \setminus U$ be the complement set of $U$ in $V(G)$, i.e.,  all literals or clauses assigned to vertices in $H$ that participate in at least one unsatisfied constraint.  We give an upper bound on the cardinality of $Q$. 
		%
		Since there are at most $\eps \cdot |E(H)|$ unsatisfied constraints, and each constraints corresponds to two vertices $x,y \in V(H)$ the number of literals assigned to vertices that participate in an unsatisfied constraint is bounded by 
		
		\begin{equation}
			\label{eq:Qq}
			\begin{aligned}
				|Q| ={} & |V(G) \setminus U| 
				\\\leq{} & \eps \cdot |E(H)| \cdot 2 \cdot \Delta(\psi)
				\\={} & \eps \cdot \left(3 \cdot |V(H)| \right)\cdot 2 \cdot \Delta(\psi)
				\\\leq{} & \eps \cdot \left(3 \cdot k \right) \cdot 2 \cdot Z \cdot \left(1+\frac{|V(G)|+|E(G)|}{k}\right) \cdot \log(k)
				\\\leq{} & \eps \cdot 6 \cdot k \cdot Z \cdot \left(1+\frac{2n+m+3 \cdot m+n}{k}\right) \cdot \log(k)
				\\\leq{} & \eps \cdot 6 \cdot k \cdot Z \cdot \left( \frac{6n+8 \cdot m}{k} \right)\cdot \log(k)
				\\\leq{} & \eps \cdot 6 \cdot Z \cdot \left(\frac{6}{\tau}+8 \right) \cdot \log(k) \cdot m 
				%	\\\leq{} &  \frac{\eps \cdot 6 \cdot Z \cdot \left(6+8 \cdot \rho \right) \cdot m \cdot \log(k) }{\tau} 
				\\={} & \frac{ \left(1-\alpha\right) \cdot m}{\rho}.  
				%O \left(\eps \cdot k \cdot \frac{n \cdot \log(k)}{k}\right) \\={} & O(\eps \cdot n \cdot \log(k)) 
				% \\={} & O(\eps' \cdot n).
			\end{aligned}
		\end{equation}
		
		Therefore,
		
		\begin{equation*}
			\label{eq:TTQ}
			\begin{aligned}
				\SAT(\phi) \geq{} & \left|  \left\{   c \in C \mid s(c[1])+s(c[2])+s(c[3]) \geq 1  \right\}  \right| 
				\\\geq{} & 	\left|\tilde{C}\right|
				\\={} &|C| - \left|  \left\{   c \in C \mid c \notin U \textnormal{ or } c[1] \notin U  \textnormal{ or } c[2] \notin U \textnormal{ or } c[3] \notin U\right\}  \right| 
				\\\geq{} & m - \rho \cdot |Q|  
					\\\geq{} & m - \rho \cdot \frac{ \left(1-\alpha\right) \cdot m}{\rho}
						\\\geq{} & m -  \left(1-\alpha\right) \cdot m
							\\={} & \alpha \cdot m
			\end{aligned}
		\end{equation*}
		By the above, the proof follows. 
	%	These clauses are all clauses without clauses in $V(G) \setminus U$ or clauses with a literal in $V(G) \setminus U$. Thus, the number of satisfied clauses by $s$ is at least $m-O( |V(G) \setminus U|) = m-O(\eps' \cdot n) = O((1-\eps') \cdot m)$ assuming $m = \Theta(n)$.%\footnote{If $m = o(n)$ then we can trivially remove all variables not participating in any clause from the problem to reach $m \geq \frac{n}{3}$.} 
	%	The above calculations can be made precise by adding suitable constants. 
	\end{claimproof}
	
	The above claims show that computing a $(1-\eps)$-approximation for $\Gamma$ can distinguish between the two cases of \Cref{thm:GAP-eth} for $\phi$. Thus, by \Cref{thm:GAP-eth}, there is no algorithm that can compute a $(1-\eps)$-approximation for $\Gamma$ in time $2^{\delta \cdot n}$.  We first give an upper bound on the encoding size of $\Gamma$.
	
		\begin{claim}
		\label{claim:EncodingG}
		$|\Gamma| \leq 2^{16 \cdot Z \cdot \left(6+8 \cdot \rho\right) \cdot \frac{n}{k}  \cdot \log(k)}$. 
	\end{claim}
	\begin{claimproof}
	For all $x \in E(H)$ it holds that 
		\begin{equation}
		\label{eq:SigmaBound}
		\begin{aligned}
		 \left|\Sigma_x\right| \leq{} & \left(|\{0,1\}|+\left|\{0,1\}\right|^3\right)^{\left|V_x(\psi)\right|}
			\\\leq{} & \left(|\{0,1\}|+\left|\{0,1\}\right|^3\right)^{\max_{x \in V(H)} \left|V_x(\psi)\right|}
			\\\leq{} &  \left(2+8\right)^{\Delta\left(\psi\right)}
			\\\leq{} &  10^{Z \cdot \left(1+\frac{|V(G)|+|E(G)|}{k}\right) \cdot \log(k)}
			\\\leq{} & 10^{Z \cdot \left(1+\frac{2n+m+3 \cdot m+n}{k}\right) \cdot \log(k)}
			\\\leq{} &  10^{Z \cdot \left( \frac{6n+8 \cdot m}{k} \right) \cdot \log(k)}
			\\\leq{} & 10^{Z \cdot \left( \frac{6n+8 \cdot \rho \cdot n}{k} \right) \cdot \log(k)}
			\\\leq{} &  2^{4 \cdot Z \cdot \left(6+8 \cdot \rho\right) \cdot \frac{n}{k}  \cdot \log(k)}
			%	\\\leq{} & 2^k \cdot 10^{\frac{n}{k} \cdot \log(k)} 
			%	\\={} & 2^k \cdot 2^{4 \cdot \frac{n}{k} \cdot \log(k)}
		\end{aligned}
	\end{equation}
	By \eqref{eq:SigmaBound} observe that the size of the alphabet of $\Gamma$ is bounded by:
	\begin{equation}
		\label{eq:SigmaBound2}
		\begin{aligned}
			|\Sigma| \leq \sum_{x \in V(H)} \left|\Sigma_x\right|
							\leq k \cdot 2^{4 \cdot Z \left(6+8 \cdot \rho\right) \cdot \frac{n}{k}  \cdot \log(k)}
		%	\\\leq{} & 2^k \cdot 10^{\frac{n}{k} \cdot \log(k)} 
		%	\\={} & 2^k \cdot 2^{4 \cdot \frac{n}{k} \cdot \log(k)}
		\end{aligned}
	\end{equation}
	%	\\\leq{} & \eps \cdot 6 \cdot k \cdot Z \cdot \left(1+\frac{2n+m+3 \cdot m+n}{k}\right) \cdot \log(k)
	%\\\leq{} & \eps \cdot 6 \cdot k \cdot Z \cdot \left( \frac{6n+8 \cdot m}{k} \right)\cdot \log(k)
	The encoding size of $H$, that is $|H|$, can be bounded by the number of vertices and edges in $H$:
	\begin{equation}
		\label{eq:EncodingH}
		|H| \leq \left|V(H)\right|+\left|E(H)\right| \leq k+3 \cdot k = 4 \cdot k.
	\end{equation}
	Finally, the encoding size of $X$, can be bounded by 
	\begin{equation}
		\label{eq:EncodingX}
		\begin{aligned}
			\sum_{(x,y) \in E(H)} \left|X_{(x,y)}\right| \leq{} & 	\sum_{(x,y) \in E(H)} \left|\Sigma_x\right| \cdot \left|\Sigma_y\right| 
			\\\leq{} & |E(H)| \cdot 2^{4 \cdot Z \cdot \left(6+8 \cdot \rho\right) \cdot \frac{n}{k}  \cdot \log(k)} \cdot 2^{4 \cdot Z \cdot \left(6+8 \cdot \rho\right) \cdot \frac{n}{k}  \cdot \log(k)} 
			\\\leq{} & 3k \cdot 2^{8 \cdot Z \cdot \left(6+8 \cdot \rho\right) \cdot \frac{n}{k}  \cdot \log(k)}. 
		\end{aligned}
	\end{equation} Therefore, by \eqref{eq:SigmaBound2}, \eqref{eq:EncodingH}, and \eqref{eq:EncodingX} the encoding size of $\Gamma$ is bounded by 
	\begin{equation*}
		\label{eq:sB2}
		\begin{aligned}
			|\Gamma| \leq{} & |H|+|\Sigma|+	\sum_{(x,y) \in E(H)} \left|X_{(x,y)}\right|  
			\\\leq{} & 4 \cdot k+ k \cdot 2^{4 \cdot Z \left(6+8 \cdot \rho\right) \cdot \frac{n}{k}  \cdot \log(k)}+3k \cdot 2^{8 \cdot Z \cdot \left(6+8 \cdot \rho\right) \cdot \frac{n}{k}  \cdot \log(k)}
				\\\leq{} &
			8 \cdot k \cdot 2^{8 \cdot Z \cdot \left(6+8 \cdot \rho\right) \cdot \frac{n}{k}  \cdot \log(k)}
				\\\leq{} &
			2^{8 \cdot \log(k)} \cdot 2^{8 \cdot Z \cdot \left(6+8 \cdot \rho\right) \cdot \frac{n}{k}  \cdot \log(k)}
				\\\leq{} &
		 2^{16 \cdot Z \cdot \left(6+8 \cdot \rho\right) \cdot \frac{n}{k}  \cdot \log(k)}
		\end{aligned}
	\end{equation*} The above equation implies the statement of the claim. 
		\end{claimproof}
	
	
	Define
	
	\begin{equation}
		\label{eq:zeta}
		\zeta =  \frac{\delta}{54 \cdot Z \cdot L \cdot \left(6+8 \cdot \rho\right) }. 
	\end{equation}
	Assume that Gap-ETH holds and assume towards a contradiction that there is an algorithm $\cA$ that given a 2-CSP instance $\Gamma' = (H',\Sigma',X')$, can decide in time $|\Gamma'0|^{\zeta \cdot \frac{r}{\log (r)}}$, where $r = |E(H)|$, whether $\CSP(\Gamma') = |E(H')|$ or $\CSP(\Gamma') < (1-\eps) \cdot |E(H')|$. Using $\cA$ we define the following algorithm $\cB$ that decides whether $\phi$ satisfies $\SAT(\phi) = m$ or $\SAT(\phi) < \alpha \cdot m$. Define $\cB$ on input $\phi$ as follows.
	
	\begin{enumerate}
		\item Compute the 2-CSP instance $\Gamma$ based on $\phi$. 
		\item Execute $\cA$ on  $\Gamma$.
		\item Return that $\SAT(\phi) = m$ if $\CSP(\Gamma) = |E(H)|$.
	\item Return that $\SAT(\phi) < \alpha \cdot m$ if $\CSP(\Gamma) < (1-\eps) \cdot |E(H)|$.
	\end{enumerate} The correctness of $\cB$ follows from \Cref{claim:completeCSP} and \Cref{claim:soundCSP}. The running time of $\cB$ on input $\phi$ is bounded by computing the instance $\Gamma$ and executing $\cA$ on input $\Gamma$. By \Cref{lem:embedding} and \Cref{def:CSP} it holds that $\Gamma$ can be computed from $\phi$ in time 
	\begin{equation}
		\label{eq:CompG}
		\begin{aligned}
			|\Gamma|+\left(|V(G)|+|E(G)|\right)^{L} \leq{} &
			 2^{16 \cdot Z \cdot \left(6+8 \cdot \rho\right) \cdot \frac{n}{k}  \cdot \log(k)}+\left(2\cdot n+m+3 \cdot m+n\right)^L
			\\\leq{} &
			 2^{16 \cdot Z \cdot \left(6+8 \cdot \rho\right) \cdot \frac{n}{k}  \cdot \log(k)}+\left(2\cdot n+\rho \cdot n+3 \cdot \rho \cdot n+n\right)^L
			 \\\leq{} &
			 2^{16 \cdot Z \cdot \left(6+8 \cdot \rho\right) \cdot \frac{n}{k}  \cdot \log(k)}+\left(3 \cdot n+4 \cdot \rho \cdot n\right)^L
			  \\\leq{} &
			 2^{16 \cdot Z \cdot \left(6+8 \cdot \rho\right) \cdot \frac{n}{k}  \cdot \log(k)}+2^{\left(3+4 \cdot \rho\right) \cdot L \cdot \log (n)}
			   \\\leq{} &
			 2^{16 \cdot Z \cdot \left(6+8 \cdot \rho\right) \cdot \frac{n}{k}  \cdot \log(k)}+2^{\left(3+4 \cdot \rho\right) \cdot L \cdot \frac{n}{k}}
			  \\\leq{} &
			 2^{17 \cdot Z \cdot L \cdot \left(6+8 \cdot \rho\right) \cdot \frac{n}{k}  \cdot \log(k)}
		\end{aligned}
	\end{equation}
	
	Hence, the running time of $\cB$ is bounded by 
	\begin{equation*}
		\label{eq:ADDw}
		\begin{aligned}
				|\Gamma|^{\left(\zeta \cdot \frac{3 \cdot k}{\log(k)}\right)}+	|\Gamma|+\left(|V(G)|+|E(G)|\right)^{L} \leq{} &  
				 \left(2^{16 \cdot Z \cdot \left(6+8 \cdot \rho\right) \cdot \frac{n}{k}  \cdot \log(k)}\right)^{\left(\zeta \cdot \frac{3 \cdot k}{\log(k)}\right)}+ 2^{17 \cdot Z \cdot L \cdot \left(6+8 \cdot \rho\right) \cdot \frac{n}{k}  \cdot \log(k)}
				 \\\leq{} &  
				 \left(2^{18 \cdot Z \cdot L \cdot \left(6+8 \cdot \rho\right) \cdot \frac{n}{k}  \cdot \log(k)}\right)^{\left(\zeta \cdot \frac{3 \cdot k}{\log(k)}\right)}
				 \\={} &  
				 2^{\zeta \cdot 54 \cdot Z \cdot L \cdot \left(6+8 \cdot \rho\right) \cdot n}
				  \\={} &  
				 2^{\delta \cdot n}. 
		\end{aligned}
	\end{equation*}
	
	\comment{
	Thus, $\Gamma$ can be computed based on $\phi,k$ in time $ O \left(2^k \cdot 2^{4 \cdot \frac{n}{k} \cdot \log(k)}\right)$ by \Cref{lem:embedding}. Moreover, the encoding size of $\Gamma$ is $N = |\Gamma| = O \left(2^k \cdot 2^{4 \cdot \frac{n}{k} \cdot \log(k)}   \right)$.  Thus, for a sufficiently small constant $\delta'$ and for $n \gg k$, by \Cref{GapETH} there is no algorithm that returns a $(1-\eps)$-approximation for $\Gamma$ in time $N^{\delta' \cdot \frac{k}{\log}}$ since:
	$$N^{\delta' \cdot \frac{k}{\log}} = \left(2^k \cdot 2^{4 \cdot \frac{n}{k} \cdot \log(k)}  \right)^{{\delta' \cdot \frac{k}{\log}}} < 2^{\delta \cdot n}.$$  
}
\end{proof}
}


==> G-CSPtoR-CSP.tex <==
\subsection{A Reduction from G-CSP to R-CSP}
\label{sec:GtoR} 

In this section, we give a straightforward reduction from G-CSP to R-CSP. This gives the proof of \Cref{thm:G-CSPtoR-CSP}. Given a G-CSP instance $\Delta =  \left(L, \{\Sigma_x\}_{x \in V(L)},\Upsilon, \{\pi_{h, x}, \pi_{h, y}\}_{h = (x,y)\in E(L)},\perp \right)$, the reduction produces an R-CSP instance $\Pi\left(\Delta\right) = \left(G,\Sigma, \mathcal{X}, \{\pi'_{e, u}, \pi'_{e, v}\}_{e = (u,v)\in E(G)},\perp' \right)$ on the same constraint graph $L = G$. In addition, the alphabet $\Sigma$ is the union of the alphabets $\Sigma_x$ for all vertices $x \in V(L)$, and the alphabet $\mathcal{X}$ consists of the (disjoint) union of the alphabet $\Upsilon$ of $\Delta$ and the vertices $V(L)$. Finally, for every $(u,v) \in E(G)$, the function $\pi'_{e, u}$ ($\pi'_{e, v}$) returns the same value as the function $\pi_{h, u}$ ($\pi_{h, v}$) on a symbol $\sigma \in \Sigma_u$ ($\sigma \in \Sigma_u$) and $'u'$ ($'v'$) otherwise. Thus, as $u \neq v$, an edge can be satisfied only if assigned values from the original alphabets of the vertices. 

%\begin{theorem} \label{thm:G-CSPtoR-CSP}
%	There is a reduction \textnormal{\textsf{G-CSP $\rightarrow $ R-CSP}} that, given a \textnormal{G-CSP} instance $\Delta$
%	returns in time $|\Delta|^{O(1)}$ an instance $\Pi(\Delta)$ of \textnormal{R-CSP} such that for all $q \in \mathbb{N}$ there is a consistent partial assignment for  $\Delta$ of size $q$ if and only if there is a consistent partial assignment for  $\Pi \left(\Delta \right)$ of size $q$. 
%\end{theorem}


The reduction is constructed as follows. Without the loss of generality, for every G-CSP instance $\Delta = \left(L, \{\Sigma_x\}_{x \in V(L)},\Upsilon, \{\pi_{h, x}, \pi_{h, y}\}_{h = (x,y)\in E(L)},\perp \right)$ assume that $\Upsilon \cap V(L) = \emptyset$. 

\begin{definition}
	\label{def:R-CSPInstance}
	Let $\Delta = \left(L, \{\Sigma_x\}_{x \in V(L)},\Upsilon, \{\pi_{h, x}, \pi_{h, y}\}_{h = (x,y)\in E(L)},\perp \right)$ be a \textnormal{G-CSP} instance. Define the {\em reduced} \textnormal{R-CSP} instance of $\Gamma$ as $\Pi\left(\Delta\right) = \left(G,\Sigma, \mathcal{X}, \{\pi'_{e, u}, \pi'_{e, v}\}_{e = (u,v)\in E(G)},\perp' \right)$ such that the following holds. 
	\begin{itemize}
		\item  Define $G = L$.
		\item Define $\Sigma = \bigcup_{x \in V(L)} \Sigma_x$. 
		\item Define $\mathcal{X} = \Upsilon \dot\cup V(L)$.  
		\item For all $e = (u,v)$ define the functions $\pi'_{e,u}: \Sigma \rightarrow \mathcal{X}$ and $\pi'_{e,v}: \Sigma \rightarrow \mathcal{X}$ as follows. For all $\sigma \in \Sigma$ define
		$$\pi'_{e,u} \left(\sigma\right) = \begin{cases}
			\pi_{e,u} \left(\sigma\right) , & \textnormal{if } \sigma \in \Sigma_u \\
			u, & \textnormal{else }
		\end{cases}$$
		Analogously, for all 
		$\sigma \in \Sigma$ define
		$$\pi'_{e,v} \left(\sigma\right) = \begin{cases}
			\pi_{e,v} \left(\sigma\right) , & \textnormal{if } \sigma \in \Sigma_v \\
			v, & \textnormal{else }
		\end{cases}$$
		\item Define $\perp' = \perp$. 
	\end{itemize}
\end{definition}


In the following, for every G-CSP instance $\Delta$, we use $\Pi\left(\Delta\right)$ to denote the R-CSP instance described in \Cref{def:R-CSPInstance}. The following lemma describes the first direction of the reduction. 

\begin{lemma} \label{lem:G-CSPtoR-CSP1}
	For every \textnormal{G-CSP} instance $\Delta$
	and $q \in \mathbb{N}$, if there is a consistent partial assignment for  $\Delta$ of size $q$ then there is a consistent partial assignment for  $\Pi \left(\Delta \right)$ of size $q$. 
\end{lemma}

\begin{proof}
	Let $\Delta = \left(L, \{\Sigma_x\}_{x \in V(L)},\Upsilon, \{\pi_{h, x}, \pi_{h, y}\}_{h = (x,y)\in E(L)},\perp \right)$ be a G-CSP instance and let $$\Pi\left(\Delta\right) = \left(G,\Sigma, \mathcal{X}, \{\pi'_{e, u}, \pi'_{e, v}\}_{e = (u,v)\in E(G)},\perp') \right)$$
	be the reduced R-CSP instance of $\Delta$ as defined in \Cref{def:R-CSPInstance}. Let $q \in \mathbb{N}$ and let
	$\varphi: V(L) \rightarrow \left(\bigcup_{x \in V(L)} \Sigma_x \cup \{\perp\} \right)$ be a consistent partial assignment for  $\Delta$ of size $q$. Define $\psi: V(G) \rightarrow \left(\Sigma \cup \{\perp\} \right)$ by $\psi(v) = \varphi(v)$ for every $v \in V(G)$. Since $G = L$ it holds that $\psi$ is well defined. Observe that $\left|\left\{ v \in V(G) \mid \psi(v) \neq \perp \right\}\right| = \left|\left\{ v \in V(L) \mid \varphi(v) \neq \perp \right\}\right| $ implying that the size of $\psi$ is $q$ since the size of $\varphi$ is $q$. It remains to show that $\psi$ is consistent. Let $e = (u,v) \in E(G)$ such that $\psi(u) \neq \perp$ and $\psi(v) \neq \perp$. Therefore, 
	by the definition of $\psi$ it holds that $\varphi(u) \neq \perp$ and $\varphi(v) \neq \perp$. Thus, by the definition of G-CSP it holds that $\varphi(u) \in \Sigma_u$ and $\varphi(v) \in \Sigma_v$. Thus, 
	$$\pi'_{e,u}(\psi(u)) = \pi_{e,u} \left(\varphi(u)\right) =  \pi_{e,v} \left(\varphi(v)\right) = \pi'_{e,v}(\psi(v))$$
	The first and last equalities hold since $\varphi(u) \in \Sigma_u$ and $\varphi(v) \in \Sigma_v$, respectively. The second equality follows from the consistency of $\varphi$ for $\Delta$ using that $\varphi(u) \neq \perp$ and $\varphi(v) \neq \perp$. By the above, the consistency of $\psi$ for $\Pi\left(\Delta\right)$ follows. 
	%	, which implies that $\psi(u) = \pi_{e,u}(\v)$ and $\varphi(v) \in \Sigma_v$
	%	, which, from the consistency of $\varphi$, implies that 
\end{proof}



\begin{lemma} \label{lem:G-CSPtoR-CSP2}
	For every \textnormal{G-CSP} instance $\Delta$
	and $q \in \mathbb{N}$, if there is a consistent partial assignment for  $\Pi\left(\Delta\right)$ of size $q$ then there is a consistent partial assignment for  $\Delta$ of size $q$. 
\end{lemma}

\begin{proof}
	Let $\Delta = \left(L, \{\Sigma_x\}_{x \in V(L)},\Upsilon, \{\pi_{h, x}, \pi_{h, y}\}_{h = (x,y)\in E(L)},\perp \right)$ be a G-CSP instance and let $$\Pi\left(\Delta\right) = \left(G,\Sigma, \mathcal{X}, \{\pi'_{e, u}, \pi'_{e, v}\}_{e = (u,v)\in E(G)},\perp') \right)$$
	be the reduced R-CSP instance of $\Delta$ as defined in \Cref{def:R-CSPInstance}. Let $q \in \mathbb{N}$ and let $\psi: V(G) \rightarrow \left(\Sigma \cup \{\perp\} \right)$ be a consistent partial assignment for  $\Pi\left(\Delta\right)$ of size $q$. For each $x \in V(L)$ fix an arbitrary $\sigma_x \in \Sigma_x$; there is such $\sigma_x$ since $\Sigma_x \neq \emptyset$ by the definition of G-CSP (see \Cref{def:G-CSPInstance}). Define 	$\varphi: V(L) \rightarrow \left(\bigcup_{x \in V(L)} \Sigma_x \cup \{\perp\} \right)$ by $$\varphi(x) = \begin{cases}
		\psi(x), & \textnormal{if } \psi(x) \in \Sigma_x \\
			\sigma_x, & \textnormal{if } \psi(x) \in \Sigma \setminus \Sigma_x \\
		\perp, & \textnormal{if } \psi(x) = \perp
	\end{cases}$$ for all $x \in V(L)$. %$\varphi(v) = \psi(v)$ for every $v \in V(L)$. %Since $G = L$ it holds that $\psi$ is well defined. 
	Observe that $\left|\left\{ v \in V(L) \mid \varphi(v) \neq \perp \right\}\right| = \left|\left\{ v \in V(G) \mid \psi(v) \neq \perp \right\}\right| $ implying that the size of $\varphi$ is $q$ since the size of $\psi$ is $q$. It remains to show that $\varphi$ is consistent. Let $e = (u,v) \in E(G)$ such that $\varphi(u) \neq \perp$ and $\varphi(v) \neq \perp$. We first show that $\varphi(u) \in \Sigma_u$ and $\varphi(v) \in \Sigma_v$. 
	
	\begin{claim}
		\label{claim:uv}
		$\varphi(u) \in \Sigma_u$ and $\varphi(v) \in \Sigma_v$. 
	\end{claim}
	\begin{claimproof}
		Since $\varphi(u) \neq \perp$ it follows that $\varphi(u) \in \Sigma$. Thus, either $\varphi(u) \in \Sigma_u$ or $\varphi(u) \in \Sigma \setminus \Sigma_u$. Assume towards a contradiction that  $\varphi(u) \in \Sigma \setminus \Sigma_u$. Thus,  $\pi'_{e,u}(\varphi(u)) = u$. Since $\varphi(u) \neq \perp$ and $\varphi(v) \neq \perp$ it follows that $\psi(u) \neq \perp$ and $\psi(v) \neq \perp$. Therefore, by the consistency of $\psi$ for $\Pi\left(\Delta\right)$ it holds that $\pi'_{e,u}(\psi(u)) = \pi'_{e,v}(\psi(v))$. However, $\pi'_{e,v}(\psi(v)) \neq u$ since either $\pi'_{e,v}(\psi(v)) \in \Sigma$ or $\pi'_{e,v}(\psi(v)) = v$, (recall that $v \neq u$ and that $\Sigma \cap V(L) = \emptyset$), implying that $\pi'_{e,u}(\psi(u)) \neq \pi'_{e,v}(\psi(v))$. We reach a contradiction  and it follows that $\varphi(u) \in \Sigma_u$. Using symmetrical arguments, it follows that $\varphi(v) \in \Sigma_v$.  
		%		This can hold only if both $\varphi(u) \in \Sigma_u$ and $\varphi(v) \in \Sigma_v$ by the definition of the functions $\pi'_{e,u}$ and $\pi'_{e,v}$. 
	\end{claimproof}
	
	Thus, using the above claim, 
	%	by the definition of $\psi$ it holds that $\varphi(u) \neq \perp$ and $\varphi(v) \neq \perp$. Thus, by the definition of G-CSP it holds that $\varphi(u) \in \Sigma_u$ and $\varphi(v) \in \Sigma_v$. Thus, 
	$$\pi_{e,u} \left(\varphi(u)\right) = \pi'_{e,u}(\psi(u)) = \pi'_{e,v}(\psi(v)) = \pi_{e,v} \left(\varphi(v)\right).$$
	The first and last equalities hold since $\varphi(u) \in \Sigma_u$ and $\varphi(v) \in \Sigma_v$, respectively, by \Cref{claim:uv}. The second equality follows from the consistency of $\psi$ for $\Pi\left(\Delta\right)$ using that $\psi(u) \neq \perp$ and $\psi(v) \neq \perp$. By the above, the consistency of $\varphi$ for $\Delta$ follows. 
	%	, which implies that $\psi(u) = \pi_{e,u}(\v)$ and $\varphi(v) \in \Sigma_v$
	%	, which, from the consistency of $\varphi$, implies that 
\end{proof}


The above lemmas directly gives the statement of the reduction. 

%$\Delta = \left(L, \{\Sigma_x\}_{x \in V(L)},\Upsilon, \{\pi_{h, x}, \pi_{h, y}\}_{h = (x,y)\in E(L)},\perp \right)$ be a \textnormal{G-CSP} instance. Define the {\em reduced} \textnormal{R-CSP} instance of $\Gamma$ as $\Pi\left(\Delta\right) = \left(G,\Sigma, \mathcal{X}, \{\pi'_{e, u}, \pi'_{e, v}\}_{e = (u,v)\in E(G)},\perp' \right)$

\subsubsection*{Proof of \Cref{thm:G-CSPtoR-CSP}:}
Given a G-CSP instance $\Delta = \Delta = \left(L, \{\Sigma_x\}_{x \in V(L)},\Upsilon, \{\pi_{h, x}, \pi_{h, y}\}_{h = (x,y)\in E(L)},\perp \right)$, where $L$ is of bounded degree $4$, the R-CSP instance $\Pi\left(\Delta\right) = \left(G,\Sigma, \mathcal{X}, \{\pi'_{e, u}, \pi'_{e, v}\}_{e = (u,v)\in E(G)},\perp' \right)$ defined in \Cref{def:R-CSPInstance} can be computed in time $|\Delta|^{O(1)}$. %Therefore, the proof follows from
The two directions of the reduction follow from \Cref{lem:G-CSPtoR-CSP1} and \Cref{lem:G-CSPtoR-CSP2}.  
In addition, it holds that 
 $\abs{V(G)} = \abs{V(L)}$ and $\abs{E(G)} = \abs{E(L)}$ and that $G$ is of bounded degree $4$ since $G = L$, using \Cref{def:R-CSPInstance}. Moreover, by \Cref{def:R-CSPInstance} it also holds that $|\Sigma| = \abs{\bigcup_{x \in V(L)} \Sigma_x}$ and $\abs{\mathcal{X}} \leq \abs{\Upsilon \cup V(L)} \leq \abs{\Upsilon} +\abs{ V(L)}$. Thus, the proof follows.   
\qed








==> Tradeoff.tex <==
\section{The Trade-off between $d$ and $\eps$ In \dkp (TBA)} 


Consider the \dkp instance of roughly $2 \cdot k$ dimensions produced by the reduction of Pasin to 2-CSP with rectangular constraints\footnote{I think that the rectangular constraints are equivalent to the classic formulation in terms of hardness of approximation.} Note that any solution to the instance have at most $2$ items with a strictly positive cost in any single dimension. Recall that the dimensions are paired up so we basically have $k$ pairs of dimensions. Moreover, the cost in each dimension is bounded by $m$ for each item.  

Let $d,\eps$ be some parameters such that $\frac{d}{\eps} \approx k \cdot \log(k)$. Let $D$ be the set of pairs of dimensions. Define an arbitrary partition $D_1,\ldots, D_d$ of $D$ such that for all $i,j \in [d]$ it holds that $|D_i| = |D_j| = \frac{k}{d}$ (up to a constant). For every $i \in [d]$ define an arbitrary bijection $\Pi_i: [|D_i|] \rightarrow D_i$. Define the following cost function $w: I \rightarrow \mathbb{N}^{d \times \{1,2\}}$ such that for every item $\ell \in I$ and pair of dimensions $i \in [d]$ define 
$$w(\ell)_{i,1} = \sum_{j \in [|D_i|]} (2 \cdot m)^j \cdot c(\ell)_{\Pi(j),1},~~~~~~~~~~w(\ell)_{i,2} = \sum_{j \in [|D_i|]} (2 \cdot m)^j \cdot c(\ell)_{\Pi(j),2}$$

For a pair of constraints $i \in [d]$, a solution can assign feasibly exactly $\frac{k}{d}$ items with positive costs in the pair of dimensions $i$ if and only if the same solution assigns exactly two items with positive costs for each pair of dimension in $D_i$. Recall that there can be at most $\frac{k}{d}$ items assigned to each constraint out of the $d$ {\em constraints}. Thus, if some constraint is not satisfies it affects at most $\frac{k}{d}$ items. Observe that a $(1-\eps)$-approximation for the instance with $d$ pairs of dimensions implies that, in the worst case removes one item from each pair of constraints. In this case, we have to multiply by $|D_i|$ the number of constraints that we {\em lose}. Thus, the number of unsatisfied pairs of constraints in $[d]$ is at most  $$\eps \cdot k \cdot \frac{k}{d} = \alpha \cdot k$$
For $\alpha = O\left(\frac{1}{\log(k)}\right)$ that satisfies the conditions of \Cref{thm:CSP} (instead of $\eps$), where recall that the optimum remains roughly $k$. Thus, we can define  $\frac{d}{\eps} = \frac{k}{\alpha}$ to make the above equation hold. By \Cref{thm:CSP} and the the reduction of Pasin there cannot be an algorithm that solves the new instance with $d$ dimensions, achieves a $(1-\eps)$-approximation in time $n^{\frac{k}{\log(k)}} = n^{\frac{d}{\eps \cdot \log^2(k)}} \approx n^{\frac{d}{\eps \cdot \log^2\left(\frac{d}{\eps}\right)}}$.  




==> auxReductions.tex <==


%\section{A Reduction from 2-CSP to VK}
%\ariel{this section should probably be entirely removed. Ilan - please verify. The content is here in a comment }
\comment{
In this section, we give the proof of \Cref{thm:redMain}. As an intermediate step in the reduction from 2-CSP to VK, we rely on the following 2-CSP variant with {\em rectangular} constraints.   

\begin{mdframed} \vspace{-0.1in}
\begin{definition} \leavevmode\vspace{-\baselineskip}
	{\bf 2-CSP with rectangular constraints (R-CSP)} 
	
	\begin{itemize}
		\item {\bf Input:} $\Pi = \left(G,\Sigma,\Upsilon, \{\pi_{e, u}, \pi_{e, v}\}_{e = (u,v)\in E(G)}\right)$
		consisting of
		\begin{itemize}
			\item A constraint graph $G$.
			\item Alphabet sets $\Sigma, \Upsilon$, where $\Upsilon = \{1,\ldots,m\}$ for some $m \in \mathbb{N}_{>0}$.  
			\item For each edge $e = (u, v) \in E(G)$, two functions $\pi_{e, u}: \Sigma \to \Upsilon$ and $\pi_{e, v}: \Sigma \to \Upsilon$.
			%\item A perpendicular symbol $\perp$ such that $\perp \notin \Sigma$.  
		\end{itemize}
		\item {\bf Consistent Partial Assignment:} For $e = (u, v) \in E(G)$, we say that that $e$ is {\em satisfied} by $(\sigma_u, \sigma_v) \in \Sigma \times \Sigma$ if and only if $\pi_{e, u}(\sigma_u) = \pi_{e, v}(\sigma_v)$. A \emph{partial assignment} is a function $\varphi: V(G) \to \Sigma \cup \{\perp\}$. %where $\Sigma = \bigcup_{v \in V(G)} \Sigma_v$, 
		%	such that for all $v \in V(G)$ it holds that $\varphi(v) \in \Sigma_v \cup \{\perp\}$. %and $\perp \notin \Sigma$. 
		%We say that 
		A partial assignment $\varphi$ is \emph{consistent} if for all $e = (u, v) \in E(G)$ such that $\varphi(u) \neq \perp$ and  $\varphi(v) \ne \perp$ it holds that $e$ is satisfied by $(\varphi(u), \varphi(v))$. The \emph{size} of the partial assignment $\varphi$ is defined as $|\varphi| := |\{v \in V(G) \mid \varphi(v) \ne \perp\}|$.
		\item {\bf Objective:} Find a consistent partial assignment of maximum size.
		%	\item  {\bf Parameter:} $k = |E(G)|$.  
	\end{itemize}
\end{definition}
\end{mdframed}

Using techniques from \cite{Marx10,karthik2023conditional}, we can show the following hardness result for R-CSP. We defer the full details to \Cref{sec:SATtoRCSP}.

\begin{theorem}
\label{thm:RCSP}
Assuming \textnormal{Gap-ETH},  there exist constants $\zeta,\beta > 0$ and $k_0 \in \N$, such that, for any constant $k \geq k_0$, there is no algorithm that takes in an \textnormal{R-CSP} instance $\Pi$ with a 3-regular constraint graph $H$ such that $|V(H)| \leq k$ variables, runs in time $O\left(|\Pi|^{\zeta \cdot \frac{k}{\log(k)}}\right)$ and distinguish between:
\begin{itemize}
\item {\bf (Completeness)} $\MaxPar(\Pi) = |V(H)|$, and,
\item {\bf (Soundness)} $\MaxPar(\Pi) < \left(1 - \frac{\beta}{\log(k)}\right) \cdot |V(H)|$.
\end{itemize}
\end{theorem} 

%The reduction from R-CSP to \dkp~is stated below. 

%The next reduction is from R-CSP to VK. %a special family of {\em flat} VK instances, in which each dimension is {\em used} by a small number of items (with non-zero cost in the dimension). We also define the {\em sparsity} of VK instances and what is a {\em tight} dimension w.r.t. a solution. 

%\begin{definition}
%	\label{def:flat}
%	Let $\cI = (I, p, d,c,B)$  be a \textnormal{VK} instance. For some $F \in \mathbb{N}$,  $\cI$ is called $F$-{\em flat} if for every solution $S$ of $\cI$ and for every dimension $j \in [d]$ it holds that $\left| \left\{ i \in S \mid c_j(i)>0 \right\}\right| \leq F$.  In addition, for some $s \in \mathbb{N}$ the instance $\cI$ is called $s$-{\em sparse} if for every $i \in I$ it holds that $\left|\left\{j \in [d] \mid c_j(i)>0\right\}\right|$. Moreover, given some solution $S$ of $\cI$ and dimension $j \in [d]$, we say that $j$ is {\em tight} for $S$ if it holds that $c_j(S) = m$. Finally, $\cI$ is called {\em uniform} if for all $i \in I$ it holds that $p(i) = 1$.
%\end{definition}

The following lemma states the reduction from R-CSP to VK %, having the additional important property that the obtained VK instance is 2-flat. The proof is given in \Cref{sec:RtoVK}.  
%MainCSPtoG-CSP,thm:red

  



\begin{lemma} 
	\label{thm:redA}
	There is a reduction \textnormal{\textsf{R-CSP $\rightarrow $ VK}} that, given an \textnormal{R-CSP} instance %with rectangular constraint instance 
	%$\Pi = (V, E, \Sigma, \{\pi_{e, u}, \pi_{e, v}\}_{e = (u,v)\in E})$ 
	$$\Pi = \left(G,\Sigma,\Upsilon, \{\pi_{e, u}, \pi_{e, v}\}_{e = (u,v)\in E(G)},\perp \right),$$
	where $G$ is of bounded degree $4$ and $F \in \left[\abs{V(G)}\right]$
	returns in time $|\Pi|^{O(1)}$ an instance $\cI(\Pi,F) = (I, p, d,c,B)$ of \textnormal{VK} such that the following holds. %the following holds.
	%
	\begin{enumerate}
		\item $3 \cdot \frac{|V(G)|+|E(G)|}{F} \leq d \leq 3 \cdot \frac{|V(G)|+|E(G)|}{F}+3$. %, where $G$ is the constraint graph of $\Pi$. 
		\item $\abs{\cI(\Pi)} = O \left(\log (|\Upsilon| \cdot F) \cdot  \abs{V(G)} \cdot \abs{ \Sigma} \cdot \left(|V(G)|+|E(G)|\right)  \right)$. %\abs{V(G)} \cdot \abs{\Sigma} \cdot \left(2 \cdot |E(G)|+|V(G)|\right) \cdot |\Upsilon|$.
		\item $W\left(\cI(\Pi,F)\right) \leq 2 \cdot F \cdot \left(3 \cdot F^2 \cdot |\Upsilon|\right)^{2 \cdot F}$. 
		
		
				\item 	If there is a consistent partial assignment to $\Pi$ of size $\abs{V(G)}$, then there is a solution for $\cI(\Pi)$ with profit $\abs{V(G)}+2 \cdot \abs{E(G)}$. 
			
				\item 	For every $q \in \mathbb{N}$, if there is a solution for $\cI(\Pi)$ of profit at least $\abs{V(G)}+2 \cdot \abs{E(G)}-q$, then there is a consistent partial assignment to $\Pi$ of size at least $\abs{V(G)} - 2 \cdot q \cdot  F$.  
				
				
				
		%if there is a consistent partial assignment to $\Pi$ of size $\abs{V(G)}$ then there is a solution for $\cI(\Pi,F)$ of profit $\abs{V(G)}+2 \cdot \abs{E(G)}$.    
		
		%$q \in \mathbb{N}$, if there is a solution for $\cI(\Pi,F)$ of profit $\abs{V(G)} +2 \cdot \abs{E(G)} - q$, then there is a consistent partial assignment to $\Pi$ of size $\abs{V(G)} - 2 \cdot q \cdot  F$.  
	\end{enumerate}
\end{lemma}




%The last remaining component in the overall reduction from 2-CSP to arbitrary, non-flat, VK instances is a reduction that takes a $2$-flat VK instance and produces a VK with a higher flat index parameter.  


%\begin{lemma} 
%	\label{lem:flatReduction}
%	There is a reduction \textnormal{\textsf{flat-VK $\rightarrow $ VK}} that, given a $2$-flat, $4$-sparse uniform \textnormal{VK} instance
%	$\cI  = (I, p, d,c,B)$ and $F \in \mathbb{N}$
%	returns in time $|\cI|^{O(1)}$ an instance $\mathcal{J}(\cI,F) = (\tilde{I}, \tilde{p}, \tilde{d},\tilde{c},\tilde{B})$ of \textnormal{VK} such that the following holds.
%	%
%	\begin{enumerate}
%		\item $\cj(\cI,F)$ is $F$-flat, $4$-sparse, and uniform.
%		\item $ \frac{d}{F} \leq \tilde{d} \leq 2 \cdot  \frac{d}{F}$. %, where $G$ is the constraint graph of $\Pi$. 
%		\item $\abs{\cj(\cI,F)} = O \left(\abs{\cI} \right)$. 
%		\item $\left(W\left(\cI\right)\right)^{\frac{d}{F}} \leq W\left(\cj(\cI)\right) \leq \left(W\left(\cI\right)\right)^{2 \cdot \frac{d}{F}}$.   
%			\item 	For every $q \in \mathbb{N}$, if there is a solution for $\cI$ of $d-q$ tight dimensions, then there is a solution for $\cj(\cI,F)$ of $\tilde{d}-q$ tight dimensions. 
%				\item 	For every $t \in \mathbb{N}$, if there is a solution for $\cj(\cI,F)$ of $\tilde{d}-t$ tight dimensions, then there is a solution for $\cI$ of $d-F \cdot t$ tight dimensions.  
%				%
%				%
%				%
%%		\item 	For every $q \in \mathbb{N}$, there is a consistent partial assignment to $\Pi$ of size $q$ if and only if there is a solution for $\cI(\Pi)$ of profit~$q$.  
%	\end{enumerate}
%\end{lemma}


Based on \Cref{thm:MainCSPtoG-CSP} and \Cref{thm:redA}, we can define a reduction from 2-CSP to VK as follows. 

\begin{definition}
	\label{def:2toVK}
	Given a \textnormal{2-CSP} instance $\Gamma = (H,\Sigma,X)$ such that $H$ is $3$-regular, let $\Pi(\Gamma)$
	be the reduced R-CSP instance of $\Gamma$. Define the {\em reduced} \textnormal{VK} instance of $\Gamma$ as $\cI(\Gamma) = \cI(\Pi(\Gamma))$ (as the reduced VK instance of the R-CSP instance $\Pi(\Gamma)$). 
\end{definition}

\pasin{I think the following is not needed anymore, and we can use \Cref{thm:redA} instead of \Cref{thm:redMain} now that we have \Cref{thm:RCSP}.}

By the above definition, we can prove \Cref{thm:redMain}.

\subsubsection*{Proof of \Cref{thm:redMain}:}

Let $\Gamma = (H,\Sigma,X)$ be a 2-CSP instance, let $$\Pi(\Gamma) = \left(G,\Sigma_{\Pi},\mathcal{X}, \{\pi_{e, u}, \pi_{e, v}\}_{e = (u,v)\in E(G)},\perp \right)$$
be the R-CSP instance described in \Cref{thm:MainCSPtoG-CSP}, and let $\cI(\Pi(\Gamma)) = (I,p,d,c,B)$ be the VK instance described in \Cref{thm:redA}.  In addition, let $k = \abs{E(H)}$. 
 We prove that $\cI(\Gamma) = \cI(\Pi(\Gamma))$ as defined in \Cref{def:2toVK} satisfies the conditions of \Cref{thm:redMain}. By \Cref{thm:MainCSPtoG-CSP} and \Cref{thm:redA} the VK instance $\cI(\Gamma)$ is constructed in time $\abs{\Gamma}^{O(1)}$. Moreover, it holds that 
\begin{equation}
	\label{eq:Iclaim}
	\begin{aligned}
		\abs{\cI(\Pi \left(\Gamma\right))} \leq{} & O \left(\abs{V(G)} \cdot \abs{\Sigma_{\Pi}} \cdot \left(2 \cdot |E(G)|+|V(G)|\right) \cdot |\mathcal{X}| \right) 
		\\\leq{} & O \left(\abs{E(H)} \cdot \abs{\Sigma}^2 \cdot \left(6 \cdot |V(H)|+ |E(H)|\right) \cdot \left(\abs{\Sigma}+\abs{V(H)} \right) \right) 
		\\\leq{} & O \left(\abs{\Gamma} \cdot \abs{\Gamma}^2 \cdot \left(6 \cdot \abs{\Gamma}+ \abs{\Gamma}\right) \cdot \left(\abs{\Gamma}+\abs{\Gamma} \right) \right) 
		\\={} & O \left(\abs{\Gamma}^5 \right). 
	\end{aligned}
\end{equation} The first inequality follows from \Cref{thm:redA}. The second inequality uses \Cref{thm:MainCSPtoG-CSP}. The third inequality holds since $V(H), E(H)$, and $\Sigma$ are part of the encoding of $\Gamma$. In addition, 
\begin{equation}
	\label{eq:Wclaim}
	\begin{aligned}
		W\left(\cI(\Pi\left(\Gamma\right))\right) \leq |\mathcal{X}| \leq \left(\abs{\Sigma}+\abs{V(H)} \right) \leq  \abs{\Gamma}. 
	\end{aligned}
\end{equation} The first inequality follows from \Cref{thm:redA}. The second inequality uses \Cref{thm:MainCSPtoG-CSP}. The third inequality holds since $V(H)$ and $\Sigma$ are part of the encoding of $\Gamma$. Additionally, note that 
\begin{equation}
	\label{eq:dBound}
	\begin{aligned}
		k  = \abs{E(H)} = \abs{V(G)} \leq \abs{V(G)}+2 \cdot \abs{E(G)} = d \leq k+2 \cdot 3 \cdot \abs{V(H)} \leq 7 \cdot k. 
	\end{aligned}
\end{equation} The second equality and the second inequality follow from \Cref{thm:MainCSPtoG-CSP}. The third equality follows from \Cref{thm:redA}.  The last inequality holds since $H$ is $3$-regular; thus, $\abs{V(H)} \leq \abs{E(H)} \leq k$. By \eqref{eq:dBound} we conclude that $k \leq d \leq 7 \cdot k$. 

It remains to prove the two directions of the reduction.
First, assume that there is an assignment for $\Gamma$ that satisfies $k = |E(H)|$ edges. Then, by  \Cref{thm:MainCSPtoG-CSP} there is a consistent partial assignment to $\Pi(\Gamma)$ of size $k$. Thus, by \Cref{thm:redA} there is a solution for $\cI  \left(\Pi \left(\Gamma\right)\right)$ of profit $k$. 
Conversely, for some $t \in \mathbb{N}$ assume that there is a solution for $\cI(\Gamma)$ of profit $k-t$. Therefore, by \Cref{thm:redA} there is a consistent partial assignment for $\Pi(\Gamma)$ of size at least $k-t$. Hence, by \Cref{thm:MainCSPtoG-CSP} there is an assignment for $\Gamma$ that satisfies at least $k-6 \cdot t$ edges. By the above, $\cI(\Gamma)$ satisfies all conditions of \Cref{thm:redMain} and the proof follows. \qed
}
 





==> generalized.tex <==


\section{2-CSP to Rectangular-CSP}
\label{sec:2toR}
In this section, we construct a reduction from 2-CSp to rectangular-CSP (R-CSP). We construct the reduction in two steps. First, we give a construction from 2-CSP to {\em generalized R-CSP (G-CSP)} - an intermediate variant of R-CSP with a different alphabet for each vertex (defined below). Second, we give a reduction from G-CSP to R-CSP and together this gives the reduction from 2-CSP to R-CSP. 

We start by formally define G-CSP. 

\begin{definition}
	\label{def:generalizedCSP}
	{\bf 2-CSP with generalized rectangular constraints (G-CSP)} 
	\begin{itemize}
		\item {\bf Input:} $\Delta = \left(L, \{\Sigma_x\}_{x \in V(L)},\Upsilon, \{\pi_{h, x}, \pi_{h, y}\}_{h = (x,y)\in E(L)},\perp \right)$
		consisting of
		\begin{itemize}
			\item A directed constraint graph $L$.
			\item Alphabet sets $\{\Sigma_x\}_{x \in V(L)}$ for every vertex of $L$ such that $\Sigma_x \neq \emptyset$ for every $x \in V(L)$.  
			\item An alphabet $\Upsilon$. 
			\item For each edge $h = (x, y) \in E(L)$, two functions $\pi_{h, x}: \Sigma_v \to \Upsilon$ and $\pi_{h, y}: \Sigma_y \to \Upsilon$. 
			\item A perpendicular symbol $\perp$ such that $\perp \notin \bigcup_{x \in V(L)} \Sigma_x$.  
		\end{itemize}
		\item {\bf Satisfied edge:} For $h = (x, y) \in E(L)$, we say that that $h$ is {\em satisfied} by $(\sigma_x, \sigma_y) \in \Sigma_x \times \Sigma_y$ if and only if $\pi_{h, x}(\sigma_x) = \pi_{h, y}(\sigma_y)$.
		
		\item {\bf Partial Assignment:} %For $h = (x, y) \in E(L)$, we say that that $h$ is {\em satisfied} by $(\sigma_x, \sigma_y) \in \Sigma_x \times \Sigma_y$ if and only if $\pi_{h, x}(\sigma_x) = \pi_{h, y}(\sigma_y)$. 
		A \emph{partial assignment} is a function $\varphi: V(L) \to \left(\bigcup_{x \in V(L)} \Sigma_x\right) \cup \{\perp\}$ such that $\varphi(x) \in \left( \Sigma_x~ \cup \perp \right)$ for every $x \in V(L)$. %where $\Sigma = \bigcup_{v \in V(G)} \Sigma_v$, 
		%	such that for all $v \in V(G)$ it holds that $\varphi(v) \in \Sigma_v \cup \{\perp\}$. %and $\perp \notin \Sigma$. 
		%We say that 
		
		\item {\bf Consistent Partial Assignment:} A partial assignment $\varphi$ is \emph{consistent} if for all $h = (x, y) \in E(L)$ such that $\varphi(x) \neq \perp$ and  $\varphi(y) \ne \perp$ it holds that $h$ is satisfied by $(\varphi(x), \varphi(y))$. 
		
		\item {\bf Size:} The \emph{size} of a partial assignment $\varphi$ is $|\{x \in V(L) \mid \varphi(x) \ne \perp\}|$.
		\item {\bf Objective:} Find a consistent partial assignment of maximum size.
		%\item  {\bf Parameter:} $k = |E(L)|$.  
	\end{itemize}
\end{definition}

The next result is our reduction from 2-CSP to G-CSP. Intuitively, given a \textnormal{2-CSP} instance 
$\Gamma = (H,\Sigma,X)$ the following reduction creates a G-CSP instance $\Delta(\Gamma)$ with the following properties. The graph $G$ of $\Delta(\Gamma)$ is the {\em line graph} of $H$ - every edge in $H$ becomes a vertex in $G$ and the edges of $G$ consist of all (lexicographically ordered) pairs of edges of $H$ with a common vertex. For each vertex of $G$ (edge of $H$) we define the alphabet of all satisfying assignment to this edge in $H$. The constraints of the instance $\Delta(\Gamma)$ require that a vertex $x$ of $H$ receives the same symbol by different vertices of $G$, or, edges of $H$, that contain $x$ as an endpoint. The proof is given in \Cref{sec:CSPtoR-CSP}. 

\begin{lemma} \label{thm:CSPtoG-CSP}
	There is a reduction \textnormal{\textsf{2-CSP $\rightarrow $ G-CSP}} that, given a \textnormal{2-CSP} instance 
	$\Gamma = (H,\Sigma,X)$ where $H$ is  $3$-regular, %the degree of each vertex in $V(H)$ is at most $4$,
	returns in time $|\Gamma|^{O(1)}$ an instance $$\Delta(\Gamma) = \left(L, \{\Sigma_x\}_{x \in V(L)},\Upsilon, \{\pi_{h, x}, \pi_{h, y}\}_{h = (x,y)\in E(L)},\perp \right)$$ of \textnormal{G-CSP} such that the following holds.
	\begin{enumerate}
		\item $|V(L)| = |E(H)|$ and $|E(L)| \leq 3 \cdot |V(H)|$. 
		\item $L$ is of bounded degree $4$. 
		\item $|\Sigma_{x}| \leq |\Sigma|^2$ %and $|\Sigma_{e}| \leq |\Sigma|^2$ 
		for every $x \in V(L)$ and $|\Upsilon| \leq |\Sigma|$. %and $h \in E(L)$. 
		\item 	%For every $q \in \mathbb{N}$, i
		If there is an assignment for $\Gamma$ that satisfies $|E(H)|$ edges then there is a consistent partial assignment to $\Delta(\Gamma)$ of size $|E(H)|$. 
		\item 	For every $t \in \mathbb{N}$, if there is a consistent partial assignment to $\Delta(\Gamma)$ of size $|E(H)|-t$, then there is an assignment for $\Gamma$ that satisfies at least $|E(H)|- 6 \cdot t$ edges.  
	\end{enumerate}
\end{lemma}

The next result is our reduction from G-CSP to R-CSP. This reduction is relatively straightforward. The proof is given in \Cref{sec:GtoR}. 

\comment{

\begin{definition}
	\label{def:R-CSPInstance}
	Let $\Delta = \left(L, \{\Sigma_x\}_{x \in V(L)},\Upsilon, \{\pi_{h, x}, \pi_{h, y}\}_{h = (x,y)\in E(L)},\perp \right)$ be a \textnormal{G-CSP} instance. Define the {\em reduced} \textnormal{R-CSP} instance of $\Gamma$ as $\Pi\left(\Delta\right) = \left(G,\Sigma, \mathcal{X}, \{\pi'_{e, u}, \pi'_{e, v}\}_{e = (u,v)\in E(G)},\perp') \right)$ such that the following holds. 
	\begin{itemize}
		\item  Define $G = L$.
		\item Define $\Sigma = \bigcup_{x \in V(L)} \Sigma_x$. 
		\item Define $\mathcal{X} = \Upsilon \dot\cup V(L)$.  
		\item For all $e = (u,v)$ define the functions $\pi'_{e,u}: \Sigma \rightarrow \mathcal{X}$ and $\pi'_{e,v}: \Sigma \rightarrow \mathcal{X}$ as follows. For all $\sigma \in \Sigma$ define
		$$\pi'_{e,u} \left(\sigma\right) = \begin{cases}
			\pi_{e,u} \left(\sigma\right) , & \textnormal{if } \sigma \in \Sigma_u \\
			u, & \textnormal{else }
		\end{cases}$$
		Analogously, for all 
		$\sigma \in \Sigma$ define
		$$\pi'_{e,v} \left(\sigma\right) = \begin{cases}
			\pi_{e,v} \left(\sigma\right) , & \textnormal{if } \sigma \in \Sigma_v \\
			v, & \textnormal{else }
		\end{cases}$$
		\item Define $\perp' = \perp$. 
	\end{itemize}
\end{definition}

}

\begin{lemma} \label{thm:G-CSPtoR-CSP}
	There is a reduction \textnormal{\textsf{G-CSP $\rightarrow $ R-CSP}} that, given a \textnormal{G-CSP} instance $$\Delta = \left(L, \{\Sigma_x\}_{x \in V(L)},\Upsilon, \{\pi_{h, x}, \pi_{h, y}\}_{h = (x,y)\in E(L)},\perp \right)$$ such that $L$  is of bounded degree $4$,
	returns in time $|\Delta|^{O(1)}$ an instance $$\Pi(\Delta) = \left(G,\Sigma, \mathcal{X}, \{\pi'_{e, u}, \pi'_{e, v}\}_{e = (u,v)\in E(G)},\perp' \right)$$ of \textnormal{R-CSP} such that the following holds.
	
	\begin{itemize}
		\item $\abs{V(G)} = \abs{V(L)}$ and $\abs{E(G)} = \abs{E(L)}$.
		\item $G$ is of bounded degree $4$. 
		 \item $|\Sigma| = \abs{\bigcup_{x \in V(L)} \Sigma_x}$. 
		\item $\abs{\mathcal{X}} \leq \abs{\Upsilon} +\abs{ V(L)}$.  
		\item For all $q \in \mathbb{N}$ there is a consistent partial assignment for  $\Delta$ of size $q$ if and only if there is a consistent partial assignment for  $\Pi \left(\Delta \right)$ of size $q$. 
	\end{itemize} 
\end{lemma}

Using \Cref{thm:CSPtoG-CSP,thm:G-CSPtoR-CSP} we can prove \Cref{thm:MainCSPtoG-CSP}.

\subsubsection*{Proof of \Cref{thm:MainCSPtoG-CSP}:}

Define a reduction \textnormal{\textsf{2-CSP $\rightarrow $ R-CSP}} as follows on a 2-CSP instance $\Gamma = (H,\Sigma,X)$ where $H$ is $3$-regular.

\begin{enumerate}
	\item Compute via \textnormal{\textsf{2-CSP $\rightarrow $ G-CSP}} the instance %$\Delta(\Gamma)$
	$$\Delta(\Gamma) = \left(L, \{\Sigma_x\}_{x \in V(L)},\Upsilon, \{\pi_{h, x}, \pi_{h, y}\}_{h = (x,y)\in E(L)},\perp \right).$$  %= \left(L, \{\Sigma_x\}_{x \in V(L)},\Upsilon, \{\pi_{h, x}, \pi_{h, y}\}_{h = (x,y)\in E(L)},\perp \right).$$
	
	\item Compute via \textnormal{\textsf{G-CSP $\rightarrow $ R-CSP}} the instance $$\Pi \left(\Delta \left(\Gamma\right)\right) = \left(G,\Sigma_{\Pi}, \mathcal{X}, \{\pi'_{e, u}, \pi'_{e, v}\}_{e = (u,v)\in E(G)},\perp' \right).$$
	
	\item Return $\Pi \left(\Delta \left(\Gamma\right)\right)$. 
\end{enumerate}
By \Cref{thm:CSPtoG-CSP,thm:G-CSPtoR-CSP} the running time of \textnormal{\textsf{2-CSP $\rightarrow $ R-CSP}} is $\abs{\Gamma}^{O(1)}$. Moreover, it holds that $V(H) = V(L) = V(G)$ and $\abs{E(G)} = \abs{E(L)} \leq 3 \cdot \abs{V(H)}$ by  \Cref{thm:CSPtoG-CSP,thm:G-CSPtoR-CSP}. In addition, it holds that $G$ is of bounded degree $4$ also by  \Cref{thm:CSPtoG-CSP,thm:G-CSPtoR-CSP}. Additionally, it holds that 
$$\abs{\Sigma_{\Pi}} = \abs{\bigcup_{x \in V(L)} \Sigma_x} \leq \sum_{x \in V(L)} |\Sigma_x| \leq \abs{V(L)} \cdot \abs{\Sigma}^2 = \abs{V(H)} \cdot \abs{\Sigma}^2.$$
The first equality follows from \Cref{thm:G-CSPtoR-CSP}. The second inequality holds by \Cref{thm:CSPtoG-CSP}. The last equality holds since $\abs{V(L)} = \abs{V(H)}$ using \Cref{thm:CSPtoG-CSP}. Furthermore, we have that 
$$\abs{\mathcal{X}} \leq \abs{\Upsilon} +\abs{ V(L)} \leq \abs{\Sigma}+\abs{V(H)}.$$
The first inequality follows from \Cref{thm:G-CSPtoR-CSP}. The second inequality holds by \Cref{thm:CSPtoG-CSP}.  It remains to prove the two directions of the reduction.

	If there is an assignment for $\Gamma$ that satisfies $|E(H)|$ edges, then by  \Cref{thm:CSPtoG-CSP} there is a consistent partial assignment to $\Delta(\Gamma)$ of size $|E(H)|$. Thus, by \Cref{thm:G-CSPtoR-CSP} there is a consistent partial assignment for  $\Pi \left(\Delta \left(\Gamma\right)\right)$ of size $|E(H)|$.  Conversely, for some $t \in \mathbb{N}$, if there is a consistent partial assignment to $\Pi \left(\Delta \left(\Gamma\right)\right)$ of size $|E(H)|-t$, then by \Cref{thm:G-CSPtoR-CSP} there is a consistent partial assignment for $\Delta(\Gamma)$ of size $|E(H)|-t$. Therefore, by \Cref{thm:CSPtoG-CSP} there is an assignment for $\Gamma$ that satisfies at least $|E(H)|- 6 \cdot t$ edges.  
\qed


\subsection{2-CSP to Generalized Rectangular 2-CSP}
\label{sec:CSPtoR-CSP}

In this section, we give a reduction from 2-CSP with bounded-degree graphs to G-CSP, the above defined %an 
intermediate variant of rectangular CSP. 
%\begin{definition}
%	\label{def:generalizedCSP}
%	{\bf 2-CSP with generalized rectangular constraints (G-CSP)} 
%	\begin{itemize}
%		\item {\bf Input:} $\Delta = \left(L, \{\Sigma_x\}_{x \in V(L)},\Upsilon, \{\pi_{h, x}, \pi_{h, y}\}_{h = (x,y)\in E(L)},\perp \right)$
%		consisting of
%		\begin{itemize}
%			\item A directed constraint graph $L$.
%			\item Alphabet sets $\{\Sigma_x\}_{x \in V(L)}$ for every vertex of $L$ such that $\Sigma_x \neq \emptyset$ for every $x \in V(L)$.  
%			\item An alphabet $\Upsilon$. 
%			\item For each edge $h = (x, y) \in E(L)$, two functions $\pi_{h, x}: \Sigma_v \to \Upsilon$ and $\pi_{h, y}: \Sigma_y \to \Upsilon$. 
%			\item A perpendicular symbol $\perp$ such that $\perp \notin \bigcup_{x \in V(L)} \Sigma_x$.  
%		\end{itemize}
%		\item {\bf Satisfied edge:} For $h = (x, y) \in E(L)$, we say that that $h$ is {\em satisfied} by $(\sigma_x, \sigma_y) \in \Sigma_x \times \Sigma_y$ if and only if $\pi_{h, x}(\sigma_x) = \pi_{h, y}(\sigma_y)$.
%		
%		\item {\bf Partial Assignment:} %For $h = (x, y) \in E(L)$, we say that that $h$ is {\em satisfied} by $(\sigma_x, \sigma_y) \in \Sigma_x \times \Sigma_y$ if and only if $\pi_{h, x}(\sigma_x) = \pi_{h, y}(\sigma_y)$. 
%		A \emph{partial assignment} is a function $\varphi: V(L) \to \left(\bigcup_{x \in V(L)} \Sigma_x\right) \cup \{\perp\}$ such that $\varphi(x) \in \left( \Sigma_x~ \cup \perp \right)$ for every $x \in V(L)$. %where $\Sigma = \bigcup_{v \in V(G)} \Sigma_v$, 
%		%	such that for all $v \in V(G)$ it holds that $\varphi(v) \in \Sigma_v \cup \{\perp\}$. %and $\perp \notin \Sigma$. 
%		%We say that 
%		
%			\item {\bf Consistent Partial Assignment:} A partial assignment $\varphi$ is \emph{consistent} if for all $h = (x, y) \in E(L)$ such that $\varphi(x) \neq \perp$ and  $\varphi(y) \ne \perp$ it holds that $h$ is satisfied by $(\varphi(x), \varphi(y))$. 
%			
%			\item {\bf Size:} The \emph{size} of a partial assignment $\varphi$ is $|\{x \in V(L) \mid \varphi(x) \ne \perp\}|$.
%		\item {\bf Objective:} Find a consistent partial assignment of maximum size.
%		%\item  {\bf Parameter:} $k = |E(L)|$.  
%	\end{itemize}
%\end{definition}
%In the following, we give the construction described in 
This gives the proof of \Cref{thm:CSPtoG-CSP}.

%For a graph $G$ and an edge $e = (u,v) \in E(G)$ let $e_1 = u$ and $e_2 = v$. Moreover, let $V[e] = \{u,v\}$ be the set of endpoints of $e$. %We note that the following reduction creates a graph with parallel edges assumed to be distinct.   


\begin{definition}
	\label{def:G-CSPInstance}
	Let $\Gamma = (H,\Sigma,X)$ be a \textnormal{2-CSP} instance where $H$ is $3$-regular. Define the {\em reduced} \textnormal{G-CSP} instance of $\Gamma$ as $$\Delta(\Gamma) = \left(L, \{\Sigma_x\}_{x \in V(L)},\Upsilon, \{\pi_{h, x}, \pi_{h, y}\}_{h = (x,y)\in E(L)},\perp \right)$$ such that the following holds. 
	\begin{itemize}
		\item  Define the {\em line} graph of $H$ as $L = (V(L),E(L))$ such that $V(L) = E(H)$ and %$E(L) = E_{\ell}(L) \cup \bigcup_{i,j \in [2]} E_{i,j}(L)$ where %$$E_{1}(L) = \left\{ ((e,1),(e,2)) \mid e \in E(H) \right\}$$ and %for all $i,j \in [2]$ define 
		%and
		$$E(L) = \big\{\left((x_1,x_2),(y_1,y_2)\right) \in V(L) \times V(L) \mid %\exists i,j \in [2] \textnormal{ s.t. } e^1_i = e^2_j\}
		|\{x_1,x_2\} \cap \{y_1,y_2\}| = 1 \textnormal{ and } (x_1,x_2) \prec (y_1,y_2)\big\}.\footnote{Recall that the operator $\prec$ relates to lexicographic order.}$$ 
		%The orientation of each $e \in E(L)$ is chosen arbitrarily. 
		\item Define $\Sigma_{x} = X_{x}$ for all $x \in V(L)$. 
		\item Define $\Upsilon = \Sigma$.  
		%\item For all $e \in V(L)$ define $\pi_{h, e^1} : \Sigma_{\Delta} \rightarrow \Upsilon_{\Delta}$
		\item Let $h = (x,y) \in E(L)$, where $x = (x_1,x_2)$ and $y = (y_1,y_2)$, and let $i,j \in [2]$ be the unique indices such that $x_i = y_j$.  %where $$, and $y = (e^2,j,2)$ for some $e^1,e^2 \in E(H)$. %, such that  $h = \left(\left(e^1,i\right),\left(e^2,j\right)\right) \in E(L)$. 
		%Define the functions $\pi_{h, x} : \Sigma_{x} \rightarrow \Upsilon$ and $\pi_{h, y} : \Sigma_{y} \rightarrow \Upsilon$ such that for all $\sigma = (\sigma_1,\sigma_2) \in \Sigma_{x}$ define $\pi_{h, x} (\sigma) = \sigma_i$ and for all $\sigma = (\sigma_1,\sigma_2) \in \Sigma_{y}$ define $\pi_{h, y} (\sigma) = \sigma_j$. 
		Define the functions $\pi_{h, x} : \Sigma_{x} \rightarrow \Upsilon$ and $\pi_{h, y} : \Sigma_{y} \rightarrow \Upsilon$ by $\pi_{h, x} (\sigma) = \sigma_i$ for every $\sigma = (\sigma_1,\sigma_2) \in \Sigma_{x}$ and $\pi_{h, y} (\sigma) = \sigma_j$ for every $\sigma = (\sigma_1,\sigma_2) \in \Sigma_{y}$. 
	\item Define $\perp$ as an arbitrary symbol such that $\perp \notin \bigcup_{x \in V(L)} \Sigma_x$. 
\end{itemize}
\end{definition}

In the following we give the main properties of the reduction. Henceforth, for every 2-CSP instance $\Gamma$, we use $\Delta\left(\Gamma\right)$ to denote the G-CSP instance described in \Cref{def:G-CSPInstance}. 

\begin{lemma}
\label{lem:GammaPi1}
Let $\Gamma = (H,\Sigma,X)$ be a \textnormal{2-CSP} instance where $H$ is $3$-regular, and let $q \in \mathbb{N}$ such that there is an assignment for $\Gamma$ that satisfies all $|E(H)|$ edges. Then, there is a consistent partial assignment to $\Delta(\Gamma)$ of size $|E(H)|$. 
\end{lemma}

\begin{proof}
Let $\lambda: V(H) \rightarrow \Sigma$ be an assignment for $\Gamma$ that satisfies all $|E(H)|$ edges and let $$\Delta(\Gamma) = \left(L, \{\Sigma_x\}_{x \in V(L)},\Upsilon, \{\pi_{h, x}, \pi_{h, y}\}_{h = (x,y)\in E(L)},\perp \right)$$ be the reduced G-CSP instance of $\Gamma$ defined in \Cref{def:G-CSPInstance}. 
%
%Define the set of vertices in $V(H)$ that satisfy all adjacent {\em in} constraints as $$S_1 = \{v \in V(H)~|~ (\lambda(u),\lambda(v)) \in X_{(u,v)} ~\forall (u,v) \in E(H)\}.$$
%Similarly, define all vertices in $V(H)$ that satisfy all adjacent {\em out} constraints by
%$$S_2 = \{u \in V(H)~|~ (\lambda(u),\lambda(v)) \in X_{(u,v)} ~\forall (u,v) \in E(H)\}.$$
%Finally, define $S = S_1 \cap S_2$ as the set of vertices that satisfy all of their adjacent constraints. 
Define $\varphi:V(L) \rightarrow \left(\bigcup_{x \in V(L)} \Sigma_x\right) \cup \{\perp\}$ by $\varphi(x) = 	\left(\lambda(x_1),\lambda(x_2)\right)$
%	 \begin{cases}
	%		\left(\lambda(x_1),\lambda(x_2)\right), & \text{if } x_1,x_2 \in S \\
	%		\perp, & \text{else } 
	%	\end{cases}$$
for all $x = (x_1,x_2) \in V(L)$. Observe that for all $x = (x_1,x_2) \in V(L)$ %it holds t $x_1,x_2 \in S$ and 
it holds that $	\left(\lambda(x_1),\lambda(x_2)\right) \in X_{x}$ since $V(L) = E(H)$ and $\lambda$ satisfies all edges in $E(H)$. %thus, $\varphi(x) = 	\left(\lambda(x_1),\lambda(x_2)\right) $ and $X_{x} = \Sigma_x$, or (ii) $\varphi(x)  = \perp$. 
Thus, for all $x \in V(L)$ it holds that 
$\varphi(x) \in \left(\Sigma_{x} ~\cup \{\perp\}\right)$ as we recall that $X_{x} = \Sigma_x$. Clearly, $$|\{x \in V(L) \mid \varphi(x) \ne \perp\}| = |V(L)| = |E(H)|.$$ Hence, the size of $\varphi$ is $|E(H)|$. It remains to prove that $\varphi$ is consistent.  
%We start by claiming the consistency of $\varphi$. 
Let $h = (x,y) \in E(L)$, where $x = (x_1,x_2)$ and $y = (y_1,y_2)$ such that $\varphi\left(x\right) \neq \perp$ and $\varphi\left(y\right) \neq \perp$ (note that this holds for every $x,y \in V(L)$). %Thus, by the definition of $\varphi$ it holds that $x_1,x_2,y_1,y_2 \in S$. Moreover, 
Observe that $x,y \in V(L)$ which implies that $x,y \in E(H)$. Therefore, it follows that $\left(\lambda(x_1),\lambda(x_2)\right) \in~X_{x}$ and $	\left(\lambda(y_1),\lambda(y_2)\right) \in X_{y}$ since $\lambda$ satisfies all edges in $E(H)$. %$x_1,x_2,y_1,y_2 \in S$. 
In addition, since $(x,y) \in E(L)$, by the definition of $E(L)$, there are unique $i,j \in [2]$ such that $x_i = y_j$. Thus, by the definition of $\pi_{h,x}$ and  $\pi_{h,y}$ it holds that 
%	\begin{equation}
	%		\label{eq:Con-R}
	%		\begin{aligned}
		%			\pi_{h,x} \left(\varphi\left(x\right)\right)
		%			 ={} &\varphi\left(x\right)_i 
		%			\\={} & \lambda(x_i) 
		%			\\={} & \lambda(y_j) 
		%			\\={} & \varphi\left(y\right)_j 
		%			\\={} & 	\pi_{h,y} \left(\varphi\left(y\right)\right) .
		%		\end{aligned}
	%	\end{equation}
\begin{equation}
	\label{eq:Con-R}
	\begin{aligned}
		\pi_{h,x} \left(\varphi\left(x\right)\right)
		=\varphi\left(x\right)_i 
		= \lambda(x_i) 
		= \lambda(y_j) 
		= \varphi\left(y\right)_j 
		= 	\pi_{h,y} \left(\varphi\left(y\right)\right),
	\end{aligned}
\end{equation}


%	\begin{equation}
	%		\label{eq:Con-R}
	%		\pi_{h,(e^1,i,1)} \left(\varphi\left((e^1,i,1)\right)\right) = \varphi\left((e^1,i,1)\right)_i = \lambda(e^1_i) = \lambda(e^2_j) = \varphi\left((e^2,j,2)\right)_j = 	\pi_{h,(e^2,j,2)} \left(\varphi\left((e^2,j,2)\right)\right) .
	%	\end{equation}
where $\varphi\left(x\right)_i$, $\varphi\left(y\right)_j$ are the $i,j$-th coordinates of the vectors $\varphi\left(x\right), \varphi\left(y\right)$, respectively. %The first and last equalities hold since $\left(\lambda(x_1),\lambda(x_2)\right) \in~X_{x}$ and $	\left(\lambda(y_1),\lambda(y_2)\right) \in X_{y}$, respectively. 
The third equality holds since %$\left(\left(e^1,i,1\right),\left(e^2,j,1\right)\right) \in E(L)$; thus, 
$x_i = y_j$. %from the definition of $E(L)$. 
By \eqref{eq:Con-R} we conclude that $\varphi$ is a consistent partial assignment for $\Delta(\Gamma)$. 
%	To conclude the proof, observe that the size of $\varphi$ satisfies
%	\begin{equation}
	%		\label{eq:sizePhi}
	%		\begin{aligned}
		%		|\{x \in V(L) \mid \varphi(x) \ne \perp\}| ={} & 	|\{(x_1,x_2) \in V(L) \mid x_1 \in S \textnormal{ and } x_2 \in S\}| 
		%		\\={} & 	
		%		 |\{(x_1,x_2) \in E(H) \mid x_1 \in S \textnormal{ and } x_2 \in S\}| 
		%		\\={} &
		%			  |E(H)|- |\{(x_1,x_2) \in E(H) \mid x_1 \notin S \textnormal{ or } x_2 \notin S\}| 
		%		\\\geq{} &
		%		  |E(H)|- 2 \cdot 4 \cdot \left(|E(H)|-q\right) 
		%		\\={} &  |E(H)|-8 \cdot \left(|E(H)|-q\right).  
		%		\end{aligned}
	%	\end{equation} The first equality follows by the definition of $\varphi$. The  inequality holds since each unsatisfied edge $e = (x_1,x_2) \in E(H)$ by $\lambda$ inflicts a removal of at most its two endpoints from $S$; since $H$ is of bounded degree $3$, every endpoint discarded from $S$ can cause at most $4$ edges to satisfy that at least one of their endpoint is not in $S$. By \eqref{eq:sizePhi} the size of $\varphi$ is at least $ |E(H)|- 8 \cdot \left(|E(H)|-q\right) $. 
	\end{proof}
	
	The following lemma gives the second direction of the reduction. 
	
	\begin{lemma}
\label{lem:GammaPi2}
Let $\Gamma = (H,\Sigma,X)$ be a \textnormal{2-CSP} instance where $H$ is $3$-regular, and let $t \in \mathbb{N}$ such that there is a consistent partial assignment to $\Delta(\Gamma)$ of size $|E(H)|-t$.  Then, there is an assignment for $\Gamma$ that satisfies at least $|E(H)|- 6 \cdot t$ edges.  
\end{lemma}

\begin{proof}
%Let $\lambda: V(H) \rightarrow \Sigma$ be an assignment for $\Gamma$ that satisfies $q$ edges and 
Let $\Delta(\Gamma) = \left(L, \{\Sigma_x\}_{x \in V(L)},\Upsilon, \{\pi_{h, x}, \pi_{h, y}\}_{h = (x,y)\in E(L)},\perp \right)$ be the reduced G-CSP instance of $\Gamma$ defined in \Cref{def:R-CSPInstance} and let $\varphi:V(L) \rightarrow \left(\bigcup_{x \in V(L)} \Sigma_{x} ~\cup \perp\right)$ be  a consistent partial assignment to $\Delta(\Gamma)$ of size $t$. Before we construct an assignment for $\Gamma$, we give some definitions. 
For all $v \in V(H)$ let $\textnormal{\textsf{Adj}}(v) = \{((u,w) \in E(H)) \mid u = v \textnormal{ or } w = v\}$ be the set of adjacent vertices to $v$ in $H$ and  let $C = \left\{u \in V(H) \mid \Adj(u) \neq \emptyset \right\}$ be all vertices with at least one adjacent edge. For all $v \in C$ choose an arbitrary {\em representative edge}  $x^v \in \Adj(v)$ and define $i_v \in [2]$ as the unique index such that $x^v_{i_v} = v$. Let $\sigma \in \Sigma$ be an arbitrary fixed symbol in the alphabet of $\Gamma$ and define an assignment $\lambda: V(H) \rightarrow \Sigma$ for $\Gamma$ by
$$\lambda(v) = \begin{cases}
	\varphi(x^v)_{i_v}, & \textnormal{if } v \in C \\
	\sigma, & \textnormal{else } 
\end{cases}$$
for all $v \in V(H)$. We remark that $\lambda$ is well defined since $x^v$ and $i_v$ are well defined for every $v \in C$. 
Define 
$$T = \left\{   v \in V(H) \mid  \varphi(x) \neq \perp \forall x \in \Adj(v)\right\}.$$
In words, $T$ is the set of all vertices in $V(H)$ whose all adjacent edges receive an assignment by $\varphi$ that is not the perpendicular symbol.  

\begin{claim}
	\label{claim:uv-in-T0}
	For all $v \in T$, $e = (v_1,v_2) \in \Adj(v)$, and $j \in [2]$ such that $v = v_j$ it holds that $$\varphi(e)_j = \varphi \left(x^v\right)_{i_v}.$$ 
\end{claim}
\begin{claimproof}
	If $e = x^v$, then $j = i_v$ and trivially $\varphi(e)_j = \varphi \left(x^v\right)_{i_v}$.  Otherwise, it holds that $x^v \neq e$. Define $$h = \begin{cases}
	\left(e,x^v\right), & \textnormal{if } e \prec x^v \\
		\left(x^v,e\right), &  \textnormal{if } x^v \prec e
	\end{cases}$$ In words, $h$ represents the pair $e,x^v$ sorted according to a lexicographic order. %$h = (e,x^v)$ %; assume without the loss
	Since $v$ is the unique common endpoint of $e$ and $x^v$, using that %$\in \Adj(x^v)$, $v \in \Adj(e)$, and 
	$x^v \neq e$, it follows that $h \in E(L)$ by \Cref{def:G-CSPInstance}. Therefore, 
	\begin{equation}
		\label{eq:claimT}
		\varphi(e)_j = \pi_{h,e}\left(\varphi\left(e\right)\right)  = \pi_{h,x^v}\left(\varphi\left(x^v\right)\right) = \varphi\left(x^v\right)_{i_v}.
	\end{equation}
	The first and last equalities hold since %$v \in \Adj(x^v)$ and $v \in \Adj(e)$ (i.e., 
	$v$ is the common vertex of the edges $e,x^v$ in $H$ using the definitions of the functions $\pi_{h,e}$ and $\pi_{h,x^v}$, respectively.  Observe that $v \in T$, implying that $\varphi(e) \neq \perp$ and $\varphi\left(x^v\right) \neq \perp$; thus, since $\varphi$ is a consistent partial assignment to $\Delta(\Gamma)$ the second equality follows. The claim follows from \eqref{eq:claimT}. 
\end{claimproof}



%	\begin{equation}
	%		\label{eq:TT}
	%		\begin{aligned}
		%			T_{1,1} ={} & \left\{    e^1_1 \in V(H) \mid  e^1 \in V(L) \textnormal{ and } \varphi\left(e^1\right) \neq \perp \textnormal{ and } \varphi\left(e^2\right) \neq \perp ~\forall \left(\left(e^1,i\right),\left(e^2,j\right)\right) \in E(L)    \right\}
		%			\\
		%			T_{1,2} ={} & \left\{    e^1_2 \in V(H) \mid  e^1 \in V(L) \textnormal{ and } \varphi\left(e^1\right) \neq \perp \textnormal{ and } \varphi\left(e^2\right) \neq \perp ~\forall \left(\left(e^1,i\right),\left(e^2,j\right)\right) \in E(L)    \right\}
		%			\\
		%			T_{2,1} ={} & \left\{    e^2_1 \in V(H) \mid  e^2 \in V(L) \textnormal{ and } \varphi\left(e^1\right) \neq \perp \textnormal{ and } \varphi\left(e^2\right) \neq \perp ~\forall \left(\left(e^1,i\right),\left(e^2,j\right)\right) \in E(L)    \right\}
		%			\\
		%			T_{2,2} ={} & \left\{    e^2_2 \in V(H) \mid  e^2 \in V(L) \textnormal{ and } \varphi\left(e^1\right) \neq \perp \textnormal{ and } \varphi\left(e^2\right) \neq \perp ~\forall \left(\left(e^1,i\right),\left(e^2,j\right)\right) \in E(L)    \right\}
		%			\\
		%			\end{aligned}
	%	\end{equation}
%\begin{equation}
%	\label{eq:TT}
%	\begin{aligned}
	%	T_{1,1} ={} & \left\{    e^1_1 \in V(H) \mid  e^1 \in V(L) \textnormal{ and } \varphi\left(e^1\right) \neq \perp \textnormal{ and } \varphi\left(e^2\right) \neq \perp ~\forall (e^1,e^2,i,j) \in E(L)    \right\}
	%	\\
	%	T_{1,2} ={} & \left\{    e^1_2 \in V(H) \mid  e^1 \in V(L) \textnormal{ and } \varphi\left(e^1\right) \neq \perp \textnormal{ and } \varphi\left(e^2\right) \neq \perp ~\forall (e^1,e^2,i,j) \in E(L)    \right\}
	%	\\
	%	T_{2,1} ={} & \left\{    e^2_1 \in V(H) \mid  e^2 \in V(L) \textnormal{ and } \varphi\left(e^1\right) \neq \perp \textnormal{ and } \varphi\left(e^2\right) \neq \perp ~\forall (e^1,e^2,i,j) \in E(L)    \right\}
	%	\\
	%	T_{2,2} ={} & \left\{    e^2_2 \in V(H) \mid  e^2 \in V(L) \textnormal{ and } \varphi\left(e^1\right) \neq \perp \textnormal{ and } \varphi\left(e^2\right) \neq \perp ~\forall (e^1,e^2,i,j) \in E(L)    \right\}
	%	\\
	%	\end{aligned}
%\end{equation}
%	and define 
%	$$T_2 = \left\{    e^2 \in V(L) \mid  \varphi\left(e^2\right) \neq \perp \textnormal{ and } \varphi\left(e^2\right) \neq \perp ~\forall (e^1,e^2,i,j) \in E(L)    \right\}.$$
%Finally, define $T = T_{1,1} \cap T_{1,2} \cap T_{1,2} \cap T_{2,2}$. In words, $T$ is the set of vertices $v \in V(H)$ such that all edges adjacent to $v$ in $E(H)$ receives an assignment different than $\perp$ by $\varphi$. %Observe that $T$ does not contain isolated vertices from $V(H)$. 
\comment{
	
	For every $v \in T$ select an arbitrary $x_v = (x^v_1,x^v_2) \in V(L)$ such that there is $i_v \in [2]$ satisfying $x^v_{i_v} = v$. %, i_v \in [2]$, and $e^v_{i_v} = v$. 
	Since $H$ is of bounded degree $3$, observe that all vertices in $T$ are endpoints of at least one edge in $E(H)$; thus, for every $v \in T$ it holds that $x^v$ and $i_v$ are well defined.  For every $v \in T$ define  $\sigma_v = 	\varphi(x^v)_{i_v}$, which is the assignment that $\varphi$ gives to vertex $v$ w.r.t. $x_v$ (note that $\varphi(x^v)_{i_v}$ is the $i_v$-th entry in the vector $\varphi(x^v)$). 
	%	$$\sigma_v = \begin{cases}
		%		\varphi(e^v)_1, & \textnormal{if } e^v_1 = v \\
		%		\varphi(e^v)_2, & \textnormal{else } 
		%	\end{cases}$$
	Since there are no isolated vertices in $T$ from $V(H)$, it holds that $\sigma_v$ is well defined for every $v \in T$. Moreover, by the definition of the alphabet $\Sigma_{x^v}$ (see \Cref{def:R-CSPInstance}) it follows that $\sigma_v \in \Sigma$ for every $v \in T$. Fix an arbitrary symbol $\sigma \in \Sigma$ and define an assignment $\lambda: V(H) \rightarrow \Sigma$ for $\Gamma$ by
	$$\lambda(v) = \begin{cases}
		\sigma_v, & \textnormal{if } v \in T \\
		\sigma, & \textnormal{else } 
	\end{cases}$$
	for all $v \in V(H)$. We remark that $\lambda$ is well defined since $\sigma_v$ is a well defined symbol from $\Sigma$ for every $v \in T$.  We use the following auxiliary claim. 
}

The above claim is used to obtain a lower bound on the number of satisfied edges by $\lambda$. 

\begin{claim}
	\label{claim:uv-in-T}
	For all $e = (u,v) \in E(H)$ such that $u,v \in T$ it holds that $\left(\lambda(u),\lambda(v) \right)  \in X_e$. 
\end{claim}
\begin{claimproof}
	Let $u,v \in T$ such that $e = (u,v) \in E(H)$. We show that $\lambda$ satisfies $e$. 
	\begin{equation}
		\label{eq:u-in-T}
		\left(\lambda(u),\lambda(v) \right) = \left(\varphi(x^u)_{i_u},\varphi(x^v)_{i_v}\right) = \left(\varphi(e)_{1},\varphi(e)_{2}\right) = \varphi\left(e\right)
	\end{equation} The first equality follows by the definition of $\lambda$ (note that $u,v \in C$ since $e \in \Adj(u) \cap \Adj(v)$). The second equality uses \Cref{claim:uv-in-T0}. 
	\comment{
		
		
		Since  $u,v \in T$ it holds that $\lambda(u) = \sigma_{u}$ and $\lambda(v) = \sigma_{v}$. By the definition of $ \sigma_{u}$ and $ \sigma_{v}$, it holds that $\sigma_u = \varphi(x^u)_{i_u}$ and  $\sigma_v = \varphi(x^v)_{i_v}$.  %$i,j \in [2]$ such that $ \sigma_{u} = \varphi \left(e^u\right)_i$ and $ \sigma_{v} = \varphi \left(e^v\right)_j$. 
		%By the definition of $\sigma_u$ and $\sigma_v$, this implies that $e^u_i = u$ and $e^v_j = v$. 
		We consider two cases.
		\begin{enumerate}
			\item $x^u = x^v$. Then, without the loss of generality, assume that $i_u = 1$ and $i_v = 2$ (clearly $u \neq v$ since $(u,v) \in E(H)$). Therefore, 
			\begin{equation}
				\label{eq:xu=xv}
				\left(\lambda(u),\lambda(v) \right) = \left(\sigma_u,\sigma_v\right) = \left(\varphi(x^u)_{i_u},\varphi(x^v)_{i_v}\right) = \left(\varphi(x^u)_{1},\varphi(x^u)_{2}\right) = \varphi\left(x^u\right)
			\end{equation} Recall that $u,v \in T$; thus, $\varphi\left(x^u\right) \in \Sigma_{e}$, which implies that $\varphi\left(x^u\right) \in \Sigma_{e}$ since $\varphi$ is a consistent partial assignment to $\Delta(\Gamma)$. It follows that  $\varphi\left(x^u\right) \in X_e$ since $\Sigma_e = X_e$. Hence, by \eqref{eq:xu=xv} it holds that   $	\left(\lambda(u),\lambda(v) \right)  \in X_e$ as required. 
			\item $x^u \neq x^v$. Therefore, it holds that $\{x^u_1,x^u_2\} \cap \{u,v\} \neq \emptyset$ and $\{x^u_1,x^u_2\} \neq \{u,v\}$; similarly, it holds that $\{x^v_1,x^v_2\} \cap \{u,v\} \neq \emptyset$ and $\{x^v_1,x^v_2\} \neq \{u,v\}$. Let $h_u = \left(x^u,e\right)$ and $h_v = \left(x^v,e\right)$. Thus, $h_u,h_v \in E(L)$ by definition. Since $u \in T$ it holds that 
			\begin{equation}
				\label{eq:u-in-T}
				\lambda(u) = \sigma_u = \varphi\left(x^u\right)_{i_u} = \pi_{h_u,x^u}\left(\varphi\left(x^u\right)\right) = \pi_{h_u,e}\left(\varphi\left(e\right)\right) = \varphi(e)_1.  
			\end{equation}
			The fourth equality holds since $\varphi$ is a consistent partial assignment for $\Delta(\Gamma)$, while $\varphi\left(x^u\right) \neq \perp$ and $\varphi\left(e\right) \neq \perp$ since $u \in T$. Analogously, 
			\begin{equation}
				\label{eq:v-in-T}
				\lambda(v) = \sigma_v = \varphi\left(x^v\right)_{i_v} = \pi_{h_v,x^v}\left(\varphi\left(x^v\right)\right) = \pi_{h_v,e}\left(\varphi\left(e\right)\right) = \varphi(e)_2.  
			\end{equation}
		}
		Therefore, by \eqref{eq:u-in-T} it holds that $	\left(\lambda(u),\lambda(v) \right) = \varphi(e)$. Since $u,v \in T$ it holds that $\varphi(e) \neq \perp$, which implies that $\varphi(e) \in \Sigma_e$ since $\varphi$ is a consistent partial assignment to $\Delta(\Gamma)$. Since $\Sigma_e = X_e$ it follows that $\left(\lambda(u),\lambda(v) \right)  \in X_e$ as required. 
		%	\end{enumerate}
\end{claimproof}

Therefore, by \Cref{claim:uv-in-T} the number of satisfied edges by $\lambda$ is at least the number of edges in $E(H)$ whose both endpoints are contained in $T$. The next claim uses the above to obtain a lower bound on the number of satisfied edges by $\lambda$. %Then,

	\begin{claim}
	\label{claim:SatisfiedEdge}
	$	\left|  \left\{   (u,v) \in E(H) \mid \left(\lambda(u),\lambda(v) \right)  \in X_e  \right\}  \right| \geq  |E(H)| - 6\cdot t$. 
\end{claim}
\begin{claimproof}
	We start with auxiliary inequalities. First, observe that the number of edges with at least one endpoint not in $T$ is bounded by 
\begin{equation}
	\label{eq:Tupd}
	\left|  \left\{   (u,v) \in E(H) \mid u \notin T \textnormal{ or } v \notin T  \right\}  \right| \leq \sum_{v \in V(H) \setminus T} \left|\Adj(v)\right| \leq 3 \cdot \left(\left|V(H)\right|-|T|\right).   
\end{equation} The first inequality holds since for each edge $(u,v) \in E(H)$ such that $u \notin T$ or $v \notin T$ there is $w \in \{u,v\}$ such that $w \in V(H) \setminus T$ and $(u,v) \in \Adj(w)$. The second inequality holds since the graph $H$ has a bounded degree $3$. Secondly, it holds that 

\begin{equation}
		\label{eq:Tupd2}
	\begin{aligned}
		|T| ={} & \left| \left\{   v \in V(H) \mid  \varphi(x) \neq \perp \forall x \in \Adj(v)\right\} \right| 
		\\={} &
		 |V(H)|- \left|\left\{ v \in V(H) \mid \exists x \in \Adj(v) \textnormal{ s.t. } \varphi(x) = \perp \right\}\right| 
		 \\\geq{} &
		 |V(H)| -  2\cdot \left|\left\{  x \in V(L) \mid \varphi(x) = \perp \right\}\right|.
	\end{aligned}
\end{equation} The inequality holds since each $x \in V(L)$ such that $\varphi(x) = \perp$ has two endpoints in $V(H)$. Therefore, 
\begin{equation*}
	\label{eq:TTQ}
	\begin{aligned}
		\left|  \left\{   (u,v) \in E(H) \mid \left(\lambda(u),\lambda(v) \right)  \in X_e  \right\}  \right| \geq{} & 	\left|  \left\{   (u,v) \in E(H) \mid u \in T \textnormal{ and } v \in T  \right\}  \right| 
		\\={} & |E(H)| - \left|  \left\{   (u,v) \in E(H) \mid u \notin T \textnormal{ or } v \notin T  \right\}  \right| 
		\\\geq{} & |E(H)| - 3 \cdot \left(|V(H)|-|T|\right) 
		\\\geq{} & |E(H)| - 3 \cdot \bigg(|V(H)|-|V(H)|+2\cdot \left|\left\{  x \in V(L) \mid \varphi(x) = \perp \right\}\right| \bigg) 
		\\={} & |E(H)| - 3 \cdot 2\cdot \left|\left\{  x \in V(L) \mid \varphi(x) = \perp \right\}\right| 
		\\={} & |E(H)| - 2 \cdot 3\cdot t
		\\={} & |E(H)| - 6\cdot t
	\end{aligned}
\end{equation*} The first inequality follows from \Cref{claim:uv-in-T}. The second inequality follows from \eqref{eq:Tupd}. %holds since each $v \in V(H) \setminus T$ has a degree at most $4$ in $H$. 
The third inequality holds by \eqref{eq:Tupd2}. By the above the proof follows. %since each $x \in V(L) = E(H)$ such that $\varphi(x) = \perp$ has only two endpoints (in $V(H)$) that cannot be in $T$.
\end{claimproof} 

 By \Cref{claim:SatisfiedEdge} the number of satisfied edges by $\lambda$ is at least $|E(H)| - 6 \cdot t$ and the proof follows. 
%$(u,v) \in E(H)$ such that $\varphi\left((u,v)\right) = \perp$ may cause the eviction of at most $u$ and $v$ from $T$; since $H$ is of bounded degree $3$, both $u$ and $v$ have at most $4$ adjacent edges in $H$, and these edges are the only edges affected by removing $u$ and $v$ from $T$. %there are at most $4$ edges connected to ea
\end{proof}



The above directly implies the correctness of the reduction. 

\subsubsection*{Proof of \Cref{thm:CSPtoG-CSP}:} Given a 2-CSP instance $\Gamma = (H,\Sigma, X)$, where $H$ is $3$-regular, the reduced instance $\Delta(\Gamma)$ can be trivially computed in time $|\Gamma|^{O(1)}$ by \Cref{def:G-CSPInstance}. It also follows from \Cref{def:G-CSPInstance} that $|V(L)| = |E(H)|$. Moreover,
\begin{equation*}
\label{eq:sB2}
\begin{aligned}
	|E(L)| ={} & \left| \big\{\left((x_1,x_2),(y_1,y_2)\right) \in V(L) \times V(L) \mid 
	|\{x_1,x_2\} \cap \{y_1,y_2\}| = 1 \textnormal{ and } (x_1,x_2) < (y_1,y_2)\big\}\right|
	\\={} & \sum_{v \in V(H)} \left|\left\{ \left(x^1,x^2\right) \in E(H) \times E(H) \mid x^1,x^2 \in \Adj(v) \textnormal{ and } x^1 \prec x^2 \right\}\right|
	\\\leq{} & \sum_{v \in V(H)} {3 \choose 2}
	\\={} & 3 \cdot |V(H)|. 
\end{aligned}
\end{equation*}

The inequality holds since $H$ is of bounded degree $3$. Thus,  $	|E(L)|  \leq 3 \cdot |V(H)|$. In addition, 
%; thus, there can be at most adjacent edges in $L$ $|E(L)| \leq {4 \choose 2} \cdot |V(H)| = 6 \cdot |V(H)|$. By definition it also holds that  $|\Sigma_{x}| \leq |\Sigma|^2$ %and $|\Sigma_{e}| \leq |\Sigma|^2$ 
for every $x \in V(L)$ it holds that $|\Upsilon| \leq |\Sigma|$. It remains to prove that $L$ is of bounded degree $4$. Let $(u,v) \in V(L)$ be a vertex in $V(L)$ (equivalently, an edge in $E(H)$). Thus, since $H$ is $3$-regular, for all $w \in \{u,v\}$ there are at most two edges $e^w_1,e^w_2 \in \Adj(w)$ such that $(u,v) \neq e^w_1,e^w_2$. Thus, there are at most $4$ edges in $E(H)$ with a common vertex in $H$ to the edge $(u,v)$. By the definition of $L$ (see \Cref{def:G-CSPInstance}), the vertex $(u,v)$ in $L$ has a degree at most $4$.
Thus,
The proof follows from \Cref{lem:GammaPi1} and \Cref{lem:GammaPi2}. \qed










==> large-factor.tex <==
\section{Large-Factor Hardness Results}


In this section, we prove our hardness results for large approximation ratio (\Cref{thm:sqrt-ratio} and \Cref{thm:sqrt-runningtime-lb}). %This is done by giving a (relatively) simple gap-preserving reduction from R-CSP to $d$-dimensional knapsack. The reduction is stated and proved below.

\begin{lemma} 
	\label{thm:red-large-gap}
	There is a reduction \textnormal{\textsf{R-CSP $\rightarrow $ VK}} that, given a \textnormal{R-CSP} instance \\
	$\Pi = \left(G,\Sigma,\Upsilon, \{\pi_{e, u}, \pi_{e, v}\}_{e = (u,v)\in E(G)},\perp \right)$, returns in time $O(|\Pi|^3)$ an instance $\cI(\Pi) = (I,p,c,B)$ of \textnormal{VK} such that the following holds.
	\begin{enumerate}
		\item $d = |V(G)| + 2|E(G)| \leq |V(G)|^2$,
		\item There is a solution for $\cI(\Gamma)$ of profit $p$ iff there is a partial assignment for $\Pi$ of size $p$.  
	\end{enumerate}
\end{lemma}

\begin{proof}
We define the instance $\cI(\Gamma)$ as follows:
\begin{itemize}
\item Let $I = V(G) \times \Sigma$, and let the profit be 1 for every item.
\item Let $d = |V(G)| + 2|E(G)|$. For notational convenience, we assume that each dimension is associated with an element in $V(G) \cup \{(e, u), (e, v) \mid e = (u, v) \in E(G)\}$.
\item Let the budget $B_j$ be $m$ for all dimensions $j$.
\item Finally, let the cost be as follows:
\begin{itemize}
\item For all $v \in V(G)$ and $\sigma \in \Sigma$, let $c_v(v, \sigma) = m$
\item For all $e = (u, v) \in E(G )$ and $\sigma \in \Sigma$, let
\begin{align*}
c_{(e, u)}(v, \sigma) &= \pi_{(e, v)}(\sigma), \\
c_{(e, v)}(v, \sigma) &= m - \pi_{(e, v)}(\sigma), \\
c_{(e, u)}(u, \sigma) &= m - \pi_{(e, u)}(\sigma), \\
c_{(e, v)}(u, \sigma) &= \pi_{(e, u)}(\sigma).
\end{align*}
\item Cost of all other items in all other coordinates are set to zero.
\end{itemize}
\end{itemize}

It is clear that the reduction runs in $O(|\Pi|^3)$ time. We next prove the completeness and soundness.

\paragraph{(Completeness)} Suppose that there is a consistent partial assignment $\varphi: V(G) \to \Sigma \cup \{\perp\}$. Then, we let the solution be $S = \{(v, \varphi(v)) \mid \varphi(v) \ne \perp\}$. Clearly, $|S| = |\varphi|$. It is also simple to verify that $S$ is a valid solution of $\cI(\Pi)$.

\paragraph{(Soundness)} Let $S \subseteq I$ be any solution of $\cI(\Pi)$. We will construct $\varphi: V(G) \to \Sigma \cup \{\perp\}$ as follows.
\begin{itemize}
\item For each $v \in V(G)$:
\begin{itemize}
\item Consider the set $\Sigma_{v, S} := \{\sigma \in \Sigma \mid (v, \sigma) \in S\}$. 
\item Observe that the coordinate $v$ implies that $|\Sigma_{v, S}| \leq 1$.
\item If $\Sigma_{v, S} = \emptyset$, let $\varphi(v) = \perp$. Otherwise, let $\varphi(v)$ be the only element in $\Sigma_{v, S}$.
\end{itemize}
\end{itemize}
It is clear that $|\varphi| = |S|$. To see that it is a consistent assignment, suppose for the sake of contradiction that this is not the case, i.e. there exists $e = (u, v) \in E(G)$ such that $\varphi(u), \varphi(v) \ne \perp$ and $\pi_{(e, u)}(\sigma) \ne \pi_{(e, v)}(\sigma)$. Suppose w.l.o.g. that $\pi_{(e, u)}(\sigma) > \pi_{(e, v)}(\sigma)$. We then have
\begin{align*}
c_{(e, v)}(v, \phi(v)) + c_{(e, v)}(u, \phi(u)) = m - \pi_{(e, v)}(\sigma) + \pi_{(e, u)}(\sigma) > m.
\end{align*}
Since $S$ contains both $(v, \phi(v))$ and $(u, \phi(u))$, it is not a valid solution to $\cI(\Pi)$, a contradiction.
\end{proof}

}

%In this section, we prove our hardness results for large approximation ratio (\Cref{thm:sqrt-ratio} and \Cref{thm:sqrt-runningtime-lb}). 

We need an initial hardness for R-CSP with a larger factor than in \Cref{thm:RCSP}. Specifically, we use the following result from \cite{chalermsook2017gap}, which shows that R-CSP is ``inherently enumerative''; putting it differently, the result states that, to distinguish the two cases, the best algorithm is essentially to straightforwardly enumerate all possible assignments to $r$ variables (which runs in time $|\Gamma|^{O(r)}$).

\begin{theorem}[\cite{chalermsook2017gap}] \label{thm:inherent-enumerate}
Assuming \textnormal{Gap-ETH}, there exist constants $\zeta > 0$ and $r_0 \in \N$, such that, for any constants $k \geq r \geq r_0$, there is no algorithm that takes in an \textnormal{R-CSP} instance $\Pi$ with a constraint graph $H$ with $|V(H)| = k$, runs in time $O\left(|\Pi|^{\zeta \cdot r}\right)$ and distinguish between:
\begin{itemize}
\item {\bf (Completeness)} $\MaxPar(\Pi) = k$, and,
\item {\bf (Soundness)} $\MaxPar(\Pi) < r$.
\end{itemize}
\end{theorem}

Since the exact statement in \cite{chalermsook2017gap} is slightly different than ours, we provide a proof of \Cref{thm:inherent-enumerate} in \Cref{sec:inherent-enumerate} for completeness.

\Cref{thm:sqrt-ratio} and \Cref{thm:sqrt-runningtime-lb} now follow directly from our reduction and \Cref{thm:inherent-enumerate} by setting appropriate parameters.

\begin{proof}[Proof of \Cref{thm:sqrt-ratio}]
Let $\zeta, r_0$ be from \Cref{thm:inherent-enumerate}. Let $r = \max\{r_0, 3C/\zeta\}, \rho = 0.5 / r$ and $d_0 = 4/\rho^2$. Suppose that there is an $(\rho \sqrt{d})$-approximation algorithm $\cA$ for $d$-dimensional knapsack that runs in $O(n^C)$ time for some $d \geq d_0$. We can use this to distinguish the two cases in \Cref{thm:inherent-enumerate} by first applying the reduction on with $k = \lfloor \sqrt{d} \rfloor$, and then run $\cA$ on the resulting instance $\cI(\Pi)$. It is simple to verify that the algorithm runs in time $O\left(|\Gamma|^{\zeta \cdot r}\right)$. Furthermore, notice that the gap between two cases is $k/r \geq \rho \sqrt{d}$. Thus, the algorithm correctly distinguishes the two cases. By \Cref{thm:inherent-enumerate}, this violates Gap-ETH.
\end{proof}

\begin{proof}[Proof of \Cref{thm:sqrt-runningtime-lb}]
Let $\zeta, r_0$ be from \Cref{thm:inherent-enumerate}. Let $\delta = \frac{\zeta}{4\rho}$ and $d_0 = (8\rho r_0)^2$. Suppose that there is an $\rho$-approximation algorithm $\cA$ for $d$-dimensional knapsack that runs in $O(n^{\delta \sqrt{d}})$ time for some $d \geq d_0$. We can use this to distinguish the two cases in \Cref{thm:inherent-enumerate} for $k = \lfloor \sqrt{d} \rfloor, r = \lfloor k / \rho \rfloor$ by first applying the reduction, and then run $\cA$ on the resulting instance $\cI(\Pi)$. It is simple to verify that the algorithm runs in time $O\left(|\Pi|^{\zeta \cdot r}\right)$. Furthermore, notice that the gap between two cases is $k/r \geq \rho$. Thus, the algorithm correctly distinguishes the two cases, which violates Gap-ETH.


\end{proof}










